Reinfier and Reintrainer: Verification and Interpretation-Driven Safe Deep Reinforcement Learning Frameworks

Ensuring verifiable and interpretable safety of deep reinforcement learning (DRL) is crucial for its deployment in real-world applications. Existing approaches like verification-in-the-loop training, however, face challenges such as difficulty in deployment, inefficient training, lack of interpretability, and suboptimal performance in property satisfaction and reward performance. In this work, we propose a novel verification-driven interpretation-in-the-loop framework Reintrainer to develop trustworthy DRL models, which are guaranteed to meet the expected constraint properties. Specifically, in each iteration, this framework measures the gap between the on-training model and predefined properties using formal verification, interprets the contribution of each input feature to the model's output, and then generates the training strategy derived from the on-the-fly measure results, until all predefined properties are proven. Additionally, the low reusability of existing verifiers and interpreters motivates us to develop Reinfier, a general and fundamental tool within Reintrainer for DRL verification and interpretation. Reinfier features breakpoints searching and verification-driven interpretation, associated with a concise constraint-encoding language DRLP. Evaluations demonstrate that Reintrainer outperforms the state-of-the-art on six public benchmarks in both performance and property guarantees. Our framework can be accessed at https://github.com/Kurayuri/Reinfier.

==> sections/Evaluation_Reinfier.tex <==
\subsection{Reinfier}

\subsubsection{Study Cases}
To evaluate the usability and effectiveness of our framework, we select the study cases utilized in related works whiRL~\cite{whiRL,whiRL_2.0} and UINT~\cite{uint} as the experimental environments.

Aurora~\cite{Aurora} is a DRL system for congestion control of TCP. It takes the latest 10 steps history of these features as input: latency inflation, latency ratio, send ratio; and it outputs the changed ratio of sending rate over the sending rate of the last action. 

Pensieve~\cite{Pensieve} is a DRL system for adaptive video bitrate selection. It takes 6 features as input: 1 value of the previous bit rate, 1 value of current buffer size, 1 value of remaining chunks, 6 values of available sizes of the next chunk, 8 values of the latest history of throughput, and 8 values of the latest history of download time; and it outputs the probability of each available bitrate of the next chunk, and the one with highest probability will be chosen as the bitrate of the next chunk.

% TODO
\input{tab/Aurora/Safety and Liveness.tex}
\input{tab/Aurora/Robustness.tex}
\subsubsection{Verification}
\input{tab/Advantage whiRL.tex}
\input{tab/Aurora/Intuitiveness Examination.tex}



\paragraph{Aurora} Four properties are proposed in whiRL~\cite{whiRL,whiRL_2.0} as follows. 

\textit{Prop 1:} When the history of local observations reflects excellent network conditions (close-to-minimum latency, no packet loss), the DNN should not get stuck at its current rate.

\textit{Prop 2:} When the history of local observations reflects excellent network conditions (close-to-minimum latency, no packet loss), the DNN should not constantly maintain or decrease its sending rate.

\textit{Prop 3:} When the congestion controller is sending on a link with a shallow buffer (and so experienced latency is always close to the minimum latency) and experiences high packet loss, it should decrease its sending rate.

\textit{Prop 4:} When the congestion controller is sending on a link with a shallow buffer (and so experienced latency is always close to the minimum latency) and consistently experiences high packet loss, it should not indefinitely maintain or increase its sending rate.


\input{tab/Aurora/Decision Boundary.tex}


We verify these properties by Reinfier but get a different result shown in Table~\ref{tab:ausl}. It has been confirmed by the authors of whiRL~\cite{whiRL} that it is a mistake in their papers after our feedback.

Here, we put forward four robustness properties for the purpose of evaluation. These properties are subsequently verified by Reinfier, and the outcomes are presented in Table~\ref{tab:aurub}. 
Prop 5 and Prop 6 are local robustness. Prop 7 describes a scenario where the input values of a single feature, i.e., send ratio, are extremely large; while Prop 8 describes a scenario where the input values of a single feature, i.e., send ratio, are abnormal behavior. This abnormal behavior is unrealistic in real-world contexts because the send ratio cannot be less than 1, which implies receiving more packages than sent ones.


\paragraph{Pensieve} 
Two properties are proposed in whiRL~\cite{whiRL,whiRL_2.0} as follows: 

\textit{Prop I:} Starting from an initial state, if chunks are downloaded quickly for a series of $k$ successive states (faster than it takes to play a chunk), the agent should eventually
not choose the worst resolution (SD).

\textit{Prop II:} Starting from an initial state, if chunks are downloaded slowly for a series of $k$ successive states (more slowly than it takes to play a chunk), the agent should eventually
not choose the highest resolution (HD).

We verify these properties by Reinfier and obtain the results consistent with whiRL's findings: specifically, Prop I does not hold, while Prop II holds.

\paragraph{Comparison}

When compared to the verification tool whiRL, our Reinfier possesses  several advantages shown in Table~\ref{tab:Advantage whiRL}. As demonstrated by the results for Aurora in Table~\ref{tab:ausl}, the error in whiRL can be attributed to the incorrect encoding of the property. This emphasizes the importance of using concise and intuitive syntax for encoding properties, which can greatly enhance the widespread and accurate application of DRL verification.

\subsubsection{Interpretability}


\begin{figure*}[!t]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]{images/DecisionBoundary/bp1bps.pkl.pdf}
    \caption{Prop 3.d}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {images/DecisionBoundary/bp2bps.pkl.pdf}
    \caption{Prop 1.a}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {images/DecisionBoundary/bp3bps.pkl.pdf}
    \caption{Prop 5.a}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/DecisionBoundary/bp4bps.pkl.pdf}
    \caption{Prop 6.a}
\end{subfigure}

\caption{Aurora Decision Boundary. The red area represents the condition where properties do not hold, while the green area represents the condition where properties hold.}
\label{fg:audb}
\end{figure*}




\paragraph{Intuitiveness Examination}

% 基于之前Aurara的Prop 3和Prop 4，我们使用Reinfier的Interpretability Module回答Intuitiveness Examination questions，对于这些性质中的一些系统边界变量进行讨论，如Table~\ref{tab:auint}所示。Prop 4.a：，它基于原本的不成立的Prop 4而来，Intuitiveness Expression： send rate越大，即丢包现象越来越严重时，更容易出现发送速率最终降低；实验结果表明，该性质在var于[1,100]的区间内，只出现的一个\textit{breakpoint}，性质由不满足转向满足，因此send rate增大更容易让发送速率最终降低，这一个性质是符合直觉的。




Based on the previous properties of Aurora, we evaluate Interpretability Module of Reinfier to answer several Intuitiveness Examination questions, as shown in Table~\ref{tab:auint}. 

\textit{Prop 4.a}: This property is derived from Prop 4. \textbf{Abstract property:} A higher send ratio, which implies more severe packet loss, is associated with a greater likelihood of the sending rate eventually decreasing. The result shows that this property only has one \text{breakpoint} for var$\in[1,100]$ following linear stepping. Within this range, the property transitions from not being satisfied to being satisfied. Consequently, this abstract property passes the intuitiveness examination.

\textit{Prop 3.a}: This property is derived from Prop 3. \textbf{Abstract property:} A higher send ratio, which implies more severe packet loss, is associated with a greater likelihood of the sending rate immediately decreasing. The result shows that this property only has one \text{breakpoint} for var$\in[1,100]$ following linear stepping. Consequently, this abstract property also passes the intuitiveness examination. Interestingly, in comparison to Prop 4.a, this result reveals that safety properties are more stringent than liveness ones for the same property structure.

\textit{Prop 3.b}: This property is derived from Prop 3. \textbf{Abstract property:} The border the constrained range of output is, which implies the more relaxed post-condition, the higher the likelihood of the property being satisfied. The result shows that this \textit{abstract} property indeed only has one \text{breakpoint} for var$\in[1,100]$ after linear search. Consequently, this abstract property also passes the intuitiveness examination. Notably, this result indicates the upper bound of the output constrained by the given input.

\textit{Prop 3.c}: This property is derived from Prop 3. \textbf{Abstract property:} A higher latency ratio, which implies higher latency, is associated with a greater likelihood of the sending rate immediately decreasing. The result shows that this property only has one \text{breakpoint} for var$\in[1,100]$ following linear stepping. Consequently, this abstract property also passes the intuitiveness examination. Besides, the result indicates that the send rate decreases only when the latency ratio is significantly high.


\begin{table*}[!t]
    \centering
    \begin{tabularx}{\textwidth}{X|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
    \hline
     & \textbf{Prop 3.d} & \textbf{Prop 1.a} & \textbf{Prop 5.b} & \textbf{Prop 6.b} 
     \\ \hline
     Type  & Safety & Liveness & Robustness & Robustness
     % \\ \hline
     % Variables 
     % & \scriptsize{a$\in[1.0,10.0]$} \newline 
     %   \scriptsize{b$\in[\phantom{0.}1,\phantom{.}100]$}
     % & \tiny{a$\in[-0.70,-0.50]$} \newline 
     %   \tiny{b$\in[\phantom{-0}1.0,\phantom{-}20.0]$}
     % & \tiny{a$\in[2.0,10.0]$} \newline 
     %   \tiny{b$\in[1.0,12.0]$}
     % & \tiny{a$\in[-0.70,-0.50]$} \newline 
     %   \tiny{b$\in[\phantom{-7}0.0,\phantom{-0}5.0]$}
     \\ \hline
    \tiny{Lower Bound and Upper Bound}\newline 
    \tiny{[latency inflation,latency ratio, send ratio]}\newline
    \scriptsize{State Boundary $S$ or Initial State $I$ }
      & \tiny {[0.00+a,1.00+b,2.00+c]} \newline [\phantom{0l+}100,\phantom{0l+}100,\phantom{0l+}100] 
      &   \tiny {[-0.01-a,\phantom{l}1.00-b,\phantom{l}1.0-c]} \newline \tiny {[\phantom{-}0.01+a,1.01+b,1.0+c]}
      &   \tiny {[0.0-a\phantom{l},1.0-b\phantom{l}, 1.0-c]} \newline  {[0.0+a,1.0+b,1.0+c]} 
      &   \tiny {[-0.7-a\phantom{l},0.5-b\phantom{l}, 1.0-c]} \newline \tiny{[-0.7+a,0.5+b, 1.0+c]} 
    \\ \hline
    Original Input $\hat{x}_0$ 
    & \multicolumn{2}{l|}{None} 
    & \scriptsize{[2.00,2.00,10.00]}
    & \scriptsize{[-0.70,0.50,1.00]}
    \\ \hline
    Original Output $N(\hat{x}_0)$ 
    & \multicolumn{2}{l|}{None} 
    & \scriptsize{-1.119}
    & \scriptsize{7.275}
    \\ \hline
    Other Condition $C$ & None &\footnotesize{No State Cycle} & None & None \\
    
    \hline
    State Transition $T$ & \multicolumn{2}{l|}{\small{History features shift by one value}}  &  \multicolumn{2}{l}{None}
    
    \\ \hline
    Post-condition $Q$ 
    & Forall \hspace{1cm} $N(x_i) < 0$ 
    & Exists \hspace{1cm} $N(x_i) \approx 0$
    & Exists \hspace{1cm} $N(x_0) > 0$
    & Exists \hspace{1cm} $N(x_0) < 0$ 
    \\ \hline
    Reinfier Result [a,b,c]  \newline
    Distance(Euclidean)    &  \small{[0.60,0.40,0.87] \newline 1.130} 
    & \small{[0.00,0.10,0.17] \newline 0.199}
    & \small{[2.20,1.20,0.16] \newline 2.511}
    & \small{[0.40,0.90,0.92] \newline 1.348}
    \\ \hline
    UINT Result [a,b,c] & \footnotesize{Not applicable} & \footnotesize{Not applicable}   & \small{[2.20,1.20,0.16] }
    & \small{[0.40,0.90,0.92]}
    \\ \hline
    
    \end{tabularx}
    \caption{Aurora Counterfactual Explanation questions and comparison of their results by Reinfier and UINT.}
    \label{tab:auce}
\end{table*}


\begin{table*}
    \centering
    \begin{tabularx}{\textwidth}{X|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
    \hline
     & \textbf{Input 1} & \textbf{Input 2} & \textbf{Input 3} & \textbf{Input 4} 
     \\ \hline
    \tiny{[latency inflation,latency ratio, send ratio]}\newline 
    \normalsize Original Input $\hat{x}_0$ 
      & \small{[0.00,1.00,1.00]} 
      & \small{[0.00,1.00,2.00]} 
      & \small{[0.00,2.00,1.00]}
      & \small{[0.00,2.00,2.00]}   \\
    \hline
     $N(x_0) \not \approx N(\hat{x_0})$ Level 1 & $\epsilon=1\times10^{-0}$ & $\epsilon=1\times10^{-0}$   & $\epsilon=1\times10^{-0}$      & $\epsilon=1\times10^{-0}$  \\
     $N(x_0) \not \approx N(\hat{x_0})$ Level 2 & $\epsilon=1\times10^{-1}$ & $\epsilon=1\times10^{-1}$   & $\epsilon=1\times10^{-1}$      & $\epsilon=1\times10^{-1}$  \\
     $N(x_0) \not \approx N(\hat{x_0})$ Level 3 & $\epsilon=1\times10^{-2}$ & $\epsilon=1\times10^{-2}$   & $\epsilon=1\times10^{-2}$      & $\epsilon=1\times10^{-2}$  \\
     $N(x_0) \not \approx N(\hat{x_0})$ Level 4 & $\epsilon=1\times10^{-3}$ & $\epsilon=1\times10^{-3}$   & $\epsilon=1\times10^{-3}$      & $\epsilon=1\times10^{-3}$  \\
    \hline
    \end{tabularx}
    \caption{Aurora Importance Analysis questions.}
    \label{tab:imau}
\end{table*}

\begin{table*}[!t]
    \centering
    \begin{tabularx}{\textwidth}{X|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
    \hline
     & \textbf{Input 1} & \textbf{Input 2} & \textbf{Input 3} & \textbf{Input 4} 
     \\ \hline
    \tiny{[latency inflation,latency ratio, send ratio]}\newline 
    \normalsize Original Input $\hat{x}_0$ 
      & \small{[0.00,1.00,1.00]} 
      & \small{[0.00,1.00,2.00]} 
      & \small{[0.00,2.00,1.00]}    
      & \small{[0.00,2.00,2.00]}   \\
    \hline
     Perturbation Level 1 & $\varepsilon=1\times10^{-0}$ & $\varepsilon=1\times10^{-0}$   & $\varepsilon=1\times10^{-0}$      & $\varepsilon=1\times10^{-0}$  \\
     Perturbation Level 2 & $\varepsilon=1\times10^{-1}$ & $\varepsilon=1\times10^{-1}$   & $\varepsilon=1\times10^{-1}$      & $\varepsilon=1\times10^{-1}$  \\
     Perturbation Level 3 & $\varepsilon=1\times10^{-2}$ & $\varepsilon=1\times10^{-2}$   & $\varepsilon=1\times10^{-2}$      & $\varepsilon=1\times10^{-2}$  \\
     Perturbation Level 4 & $\varepsilon=1\times10^{-3}$ & $\varepsilon=1\times10^{-3}$   & $\varepsilon=1\times10^{-3}$      & $\varepsilon=1\times10^{-3}$  \\
    \hline
    \end{tabularx}
    \caption{Aurora Sensitivity Analysis questions.}
    \label{tab:seau}
\end{table*}

\paragraph{Decision Boundary}
% \begin{table*}[!t]
%     \centering
%     \begin{tabularx}{0.8\textwidth}{X|p{2cm}|p{2cm}|p{2cm}}
%     \hline
%      & \textbf{Prop 3.d} & \textbf{Prop 1.a} &  \textbf{Prop 6.a} 
%     \\ \hline
%      Type  & Safety & Liveness  & Robustness
%      \\ \hline
%      Variables 
%      & \scriptsize{a$\in[1.0,10.0]$} \newline 
%        \scriptsize{b$\in[\phantom{0.}1,\phantom{.}100]$}
%      & \tiny{a$\in[-0.70,-0.50]$} \newline 
%        \tiny{b$\in[\phantom{-0}1.0,\phantom{-}20.0]$}
%      & \tiny{a$\in[-0.70,-0.50]$} \newline 
%        \tiny{b$\in[\phantom{-7}0.0,\phantom{-0}5.0]$}
%      \\ \hline
%     \tiny{Lower Bound and Upper Bound}\newline 
%     \tiny{[latency inflation,latency ratio, send ratio]}\newline
%     \scriptsize{State Boundary $S$ or Initial State $I$ }
%       & \scriptsize {[\phantom{oo}a,\phantom{oo}b,\phantom{oo}2]} \newline [100,100,100] 
%       & \scriptsize {[a,b,1]} \newline [a,b,1] 

%       &  \scriptsize {[a-$\varepsilon$,b-$\varepsilon$,1.00]}  [a+$\varepsilon$,b+$\varepsilon$,1.00]   
%       $\varepsilon=0.005$
%     \\ \hline
%     Original Input $\hat{x}_0$ 
%     & \multicolumn{2}{l|}{None} 
%     & \scriptsize{[-0.70,0.50,1.00]}
%     \\ \hline
%     Other Condition $C$ & None &\footnotesize{No State Cycle}  & None \\
    
%     \hline
%     State Transition $T$ & \multicolumn{2}{l|}{\small{History features shift by one value}}  &  None
    
%     \\ \hline
%     Post-condition $Q$ 
%     & Forall \hspace{1cm} $N(x_i) < 0$ 
%     & Exists \hspace{1cm} $N(x_i) > 0$
%     & \scriptsize{$N(x_0)\approx N(\hat{x}_0)$} \scriptsize{$\epsilon=0.5$} 
   
%     \\ \hline
    
%     \end{tabularx}
%     \caption{Aurora Decision Boundary Questions}
%     \label{tab:aubd}
% \end{table*}

Based on the previous properties of Aurora, we opt for one safety, one liveness, and two robustness properties to analyze their decision boundaries, detailed in Table~\ref{tab:aubd}. In the case of safety and liveness, the decision boundary delineates the condition where the agent takes safe or lively actions. As long as the environmental state falls within the specified space, the agent's actions align with the desired properties, averting unforeseen actions. 

The results shown in Figure \ref{fg:audb} reveal that, within the designated range, the decision boundaries for safety and liveness properties are \textit{linear}, effectively partitioning the input space into two regions: one where the property holds and another where not. Conversely, the decision boundary for the robustness property is \textit{coarse}, segmenting the input space into three distinct zones: a central area where the property holds, flanked by two regions where not.

\paragraph{Counterfactual Explanation}
Based on the previous properties of Aurora, we conduct the searches for the closest counterexamples that lead to altered verification results. The questions posed and their results are illustrated in Table~\ref{tab:auce}. Taking Prop 5.b derived from Prop 5 as an example, the original output is -1.119; thus, it proves valuable to seek a counterexample input resulting in an output greater than 0. Remarkably, the result demonstrates that the Euclidean distance to the closest counterexample amounts to 2.511.

Indeed, as outlined in the Counterfactual Explanation section of the main text, this approach can also be applied to safety and liveness properties. For instance, consider Prop 1.a derived from Prop 1, and since Prop 1 is verified to be satisfied, we can proceed to search for its counterexamples. In this case, we are interested in finding inputs where the output is approximately 0, and we can gain insights into the conditions under which the sending rate might remain unchanged.

% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.16\textwidth}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 1}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Importance/1.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 2}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Importance/2.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 3}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Importance/3.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 4}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Importance/4.0.pdf}
%     \caption{Level 1}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Importance/1.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/2.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/3.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/4.1.pdf}
%     \caption{Level 2}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Importance/1.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/2.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/3.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/4.2.pdf}
%     \caption{Level 3}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Importance/1.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/2.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/3.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/4.3.pdf}
%     \caption{Level 4}
% \end{subfigure}
% \begin{subfigure}[t]{0.32\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Importance/1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Importance/4.pdf}
%     \caption{Importance}
% \end{subfigure}
% \caption{Aurora Importance Analysis Results. Each row indicates different original input $\hat{x}_0$ as shown in Table~\ref{tab:imau}. The first to fourth columns indicate different $N(x_0) \not \approx N(\hat{x_0})$ Levels as shown in Table~\ref{tab:imau}, and the fifth column indicates the proportion of Importance ($1/Perturbation\ value$) of each feature under the three features of the input.}
% \label{fg:auim}
% \end{figure*}

\begin{figure*}[!t]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {images/Importance/1.pdf}
    \caption{Input 1}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Importance/2.pdf}
    \caption{Input 2}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Importance/3.pdf}
    \caption{Input 3}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Importance/4.pdf}
    \caption{Input 4}
\end{subfigure}
\caption{Aurora Importance Analysis Results. 
% Each row indicates different original input $\hat{x}_0$ as shown in Table~\ref{tab:imau}. The first to fourth columns indicate different $N(x_0) \not \approx N(\hat{x_0})$ Levels as shown in Table~\ref{tab:imau}, and
% the fifth column indicates 
The proportion of Importance ($1/Perturbation\ value$) of each feature under the three features of the input.}
\label{fg:auim}
\end{figure*}


% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.16\textwidth}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 1}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/1.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 2}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/2.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 3}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/3.0.pdf}
%     \makebox[0pt][r]{\makebox[30pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{Original Input 4}}}}%
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/4.0.pdf}
%     \caption{Level 1}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Sensitivity/1.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/2.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/3.1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/4.1.pdf}
%     \caption{Level 2}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Sensitivity/1.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/2.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/3.2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/4.2.pdf}
%     \caption{Level 3}
% \end{subfigure}
% \begin{subfigure}[t]{0.16\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Sensitivity/1.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/2.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/3.3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/4.3.pdf}
%     \caption{Level 4}
% \end{subfigure}
% \begin{subfigure}[t]{0.32\textwidth}
%     \includegraphics[width=\textwidth]  
%     {images/Sensitivity/1.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/2.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/3.pdf}
%     \includegraphics[width=\textwidth]
%     {images/Sensitivity/4.pdf}
%     \caption{Sensitivity}
% \end{subfigure}

% \caption{Aurora Sensitivity Analysis Results. Each row indicates different original input $\hat{x}_0$ as shown in Table~\ref{tab:seau}. The first to fourth columns indicate different Perturbation Levels as shown in Table~\ref{tab:seau}, and the fifth column indicates the proportion of Sensitivity ($Output\ deviation$) of each feature under the three features of the input.}
% \label{fg:ause}
% \end{figure*}


\begin{figure*}[!t]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {images/Sensitivity/1.pdf}
    \caption{Input 1}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Sensitivity/2.pdf}
    \caption{Input 2}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Sensitivity/3.pdf}
    \caption{Input 3}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]  
    {images/Sensitivity/4.pdf}
    \caption{Input 4}
\end{subfigure}
\caption{Aurora Sensitivity Analysis Results.
 % Each row indicates different original input $\hat{x}_0$ as shown in Table~\ref{tab:seau}. The first to fourth columns indicate different Perturbation Levels as shown in Table~\ref{tab:seau}, and the fifth column indicates 
 The proportion of Sensitivity ($Output\ deviation$) of each feature under the three features of the input.}
\label{fg:ause}
\end{figure*}

\paragraph{Importance Analysis}

\input{tab/Advantage UINT.tex}

Indeed, the assessment of feature importance can be influenced by how "output changes" are defined. In cases where the output is a floating-point number, like in Aurora, defining the extent of change in $N(x_0)$ compared to $N(\hat{x}_0)$ becomes crucial. To address this, four different levels of defining "change", i.e., $N (x_0) \not \approx N(\hat{x} _0) \equiv (N(x_0)\ge N(\hat{x} _0)) \vee (N(x_0)\le N(\hat{x} _0)) $, have been adopted. This approach provides a range of criteria for determining change and has been applied to four original inputs $\hat{x}_0$, as detailed in Table~\ref{tab:imau}.

% The importance of features, which is measured by the amount of perturbation required on the input features to change the output, may vary depending on the definition of "the output changes". Some features with small perturbation can also lead to small changes in the output, but large perturbation cannot cause large changes in the output, while others have the opposite. The output is an integer, such as classification problems, there will be no such doubt. But since Aurora's output is a float number, it is necessary to define the degree of $N (x_0) \not \approx N(\hat{x} _0)$. Therefore, we adopt four different levels of defining "change", i.e., $N (x_0) \not \approx N(\hat{x} _0) \equiv N(x_0)\ge N(\hat{x} _0) \vee N(x_0)\le N(\hat{x} _0) $ and take four original inputs $\hat{x}_0$, as shown in Table~\ref{tab:imau}.

The evaluation results are shown in Fig.~\ref{fg:auim}. They illustrate that under the four different original inputs discussed, small perturbations of latency inflation lead to output changing, and the required perturbation values are much less than the other two features.
The relationship between the importance of latency ratio and send ratio varies depending on the original input context. However, in the chosen experimental settings, the diverse definitions of $N(x_0) \not \approx N(\hat{x}_0)$ do not substantially affect the relative importance relationship between the required perturbation values for these three features.

To quantify feature importance, the reciprocal of the perturbation value is employed as the measure of importance. The results illustrate that latency inflation stands out as the most crucial feature in decision-making under these circumstances. This is likely attributed to the fact that the selected original inputs have latency inflation values close to 0, indicating network latency stability. As a result, even a slight perturbation to latency inflation might signify a shift to an unstable network latency condition, prompting the agent to significantly adjust its sending rate.


\paragraph{Sensitivity Analysis}

The sensitivity of features, as measured by the deviation of the output from its original value, varies based on the chosen perturbation levels for the features. To comprehensively analyze this, we employ four different perturbation levels denoted by $\varepsilon$ and utilize the same set of four original inputs $\hat{x}_0$ that were used in the Importance Analysis. The perturbation levels, as well as the corresponding original inputs, are listed in Table~\ref{tab:seau}. This approach helps us to explore how different perturbation levels influence the sensitivity of the features under evaluation.

The evaluation results are shown in Fig.~\ref{fg:ause}. They reaffirm the finding that perturbing latency inflation has the most substantial impact on the output, consistent with the observations from the Importance Analysis. Therefore, latency inflation remains the most sensitive feature under the given original inputs. This correlation between importance and sensitivity is reasonable, as features that are important tend to exhibit higher sensitivity due to their significant influence on the output. The high sensitivity of latency inflation suggests that slight variations in network latency can lead to noticeable changes in the agent's decision-making. This aligns with the notion that changes in latency may indicate shifts in network stability, prompting the agent to adjust its sending rate accordingly.

\paragraph{Comparison}
When compared to the interpretability tool UINT, our Reinfier possesses several advantages shown in Table~\ref{tab: Advantage UINT}. Beyond its benefits in terms of user-friendliness and applicability to a wide range of scenarios, a crucial aspect is our conviction that our unified solutions based on \textit{breakpoints} can be rapidly adapted to new interpretability problems instead of formulating distinct solutions for each individual problem. While the process of searching for \textit{breakpoints} might be time-consuming, once these breakpoints are identified, an array of interpretable problems can be answered within seconds. This further underscores the scalability of our solutions.




==> sections/FutureWork.tex <==
\section{Limitations and Future Work}
% Regarding Reinfier, addressing the issue of lengthy DRL verification times is crucial, necessitating the improvement of verification speed and responsiveness. The concept of incremental verification becomes particularly relevant for DRL systems that continue to learn even after deployment. Moreover, there is a significant research opportunity in systematically and comprehensively defining the properties of DRL.
% For Reintrainer, the current training feedback process's exclusive reliance on reward shaping proves effective for simpler properties but might fall short for more intricate ones. Drawing inspiration from curriculum learning~\cite{CL}, where the training environment evolves to target the model's shortcomings, integrating such an approach could enhance Reintrainer's performance. 
For multi-step properties, \rf~itself cannot address stochasticity or unknown environments as related works~\cite{whiRL,whiRL_2.0,verisig2.0,trainify}, which might limit its application scenarios; the former can be alleviated through over-approximation\cite{overapproximation}, while the latter can be addressed by environment modeling; and the lengthy verification time necessitates the improvement of verification techniques, like incremental verification. Besides, the current integration with reward shaping proves effective for simpler properties but might fall short for more intricate ones, thus integrating our framework with constrained optimization-based algorithms could enhance performance. 

==> sections/ReinfierBack.tex <==
\section{Design of Reinfier}

\begin{figure*}[!b]
\centering
\includegraphics[width=\textwidth]{images/Reinfier.pdf}
\caption{Working procedure of Reinfier. }
\label{Reinfier}
\end{figure*}
As a key component of \rt, we design and implement \rf~as the backend for verification and interpretation, which achieves functions far beyond \rt's requirements and also addresses \yzx{challenges of reusability and completeness in terms of the property type as well as the interpretability question type}. Therefore, it can also be used as an independent and user-friendly tool for DRL verification and interpretation.
% \rf~ is aimed at assisting designers of DRL systems effectively and effortlessly to know whether their trained models are safe or robust and how their models make decisions. 
% Therefore, \rf~ is implemented to provide numerous user-friendly interfaces to facilitate verification and interpretability of DRL through the utilization of DRLP.

Fig.~\ref{Reinfier} shows the working procedure of \rf. To avoid reinventing the wheel, fully utilize the developments in the DNN formal verification field, and maintain good scalability, we opt to use existing DNN verifiers DNNV~\cite{DNNV} and Verisig~\cite{verisig} as the verification backend for DNN. In \rf, we design and implement a parser for given DRLP properties, and an adapter for given DNN models. \jiaqi{These components act as middleware for \rf~and DNN verifiers.}\yzx{These components function as intermediaries, bridging Reinfier with the DNN verifiers.} We implement the single verifier through model checking or using reachability analysis, obtaining traditional Boolean DRL verification results (whether properties hold or not) derived from previous DRL verification works~\cite{whiRL,verisig}.
Building upon this foundation, we introduce novel concepts and methods, including \textsl{batch verification} to obtain numeric DRL verification results (under what circumstances properties hold or where not), which addresses the challenge of \textsl{concretizing} the qualitative \textsl{abstract property} into quantitative ones and are more accurate on evaluating how safe and robust the DRL model is. Additionally, we propose \textit{breakpoints} searching, providing insights into the decision boundaries of the model. Finally, we design a breakpoint-based interpreter to answer interpretability questions and understand the DRL system.

In the main text, we introduce novel concepts and methods, while the detailed functional design is provided in Appendix~\ref{Appx:Reinfier}.







% For a single DRL verification query, Verification Algorithm Module of \rf~ takes a DRLP property, a DNN and the name of a DNN verifier (optional, which can be selected by Verifier Selection Module) as inputs; then, the module oversees DRLP Translation Module as well as DNN Unrolling Module to transform these inputs into the forms for external DNN Verification Framework and run a single DNN verification query; later, the module decides whether to continue or give final verification result in a standardized format based on the DNN query result. Note that in a single DRL verification query, multiple DNN verification queries may be executed. For Verification \& Interpretability Extension Module, it takes an \textit{abstract} DRLP property which can be used for \textit{batch verification} or interpretability questions, and a DNN as inputs; it runs many DRL verification queries by calling Verification Algorithm Module multiple times.

% \begin{figure}[!b]
% \centering
% \includegraphics[width=\linewidth]{images/UnrolledDNN.pdf}
% \caption{A toy DRL system (top) is encoded for verification with depth $k=3$ (bottom).} \label{UnrolledDNN}
% \end{figure}

% \subsection{Auxiliary Modules}
% \paragraph{DNN Unrolling Module}
% Due to the multiple interactions between the agent and the environment, all constraints from the property and the DRL system as well as the DNN need encoding to be consistent with verification depth $k$. As shown in Fig.~\ref{UnrolledDNN}, the agent DNN (top) is unrolled and encoded 3 times larger (bottom) than the original when verification depth $k=3$. This unrolled DNN is used as the input DNN for DNN verification. 
% $x_i^j$ denotes the $j$-th value of the input of the $i$-th original DNN; the input of the $i$-th original DNN $x_i=\langle x_i^0,...,x_i^{n-1} \rangle$; the input $x=\langle x_0,...,x_{k-1} \rangle$.
% $y_i^j$ denotes the $j$-th value of the output of the $i$-th original DNN; the output of the $i$-th original DNN $y_i=\langle y_i^0,...,y_i^{m-1} \rangle$; the output $y=\langle y_0,...,y_{k-1} \rangle$.

% \paragraph{Verifier Selection Module}
% For supporting several DNN verifiers~\cite{Marabou,Neurify,nnenum,Planet} well, if no verifier is specified, \rf~ will select the verifier with the minimum total time that is runnable on the given DNN and DRLP in verification depth $k=1$ and $k=2$.

\subsection{Descriptive Language: DRLP}
% Due to the lack of a standard format for encoding DRL properties, we design DRLP and implement the corresponding parser. DRLP allows for a significantly more intuitive and expressive description of DRL properties. Beyond verification tasks, DRLP can be employed to effectively encode interpretability questions answered by \rf~. Furthermore, DRLP facilitates the seamless integration of property constraints as well as results of verification and interpretability questions into the training process of DRL models.

We present a descriptive language DRLP and the detailed syntax is defined in Appendix~\ref{Appx:DRLP}.
All the properties and the trained DRL system need to be encoded using DRLP as a verification script. 
% Besides $\bm{S},\bm{T},\bm{I}$ defined in DRL systems, four parts including Other condition $\bm{C}$  should be encoded in pre-condition $P$.

%\textbf{Pre-condition $\bm{P}$} is divided into four parts in DRLP:
%\textbf{State space condition $\bm{S}$}, 
% the boundary of the environment in DRL. 
%and all input variables should be bounded.
%\textbf{Initial state condition $\bm{I}$}, 
% the initial state of the system.
% , because a DRL system could start from a defined state or within a particular state boundary.
% However, what needs to be verified sometimes is that the system starts from any initial state within $S$, in which case $I$ defaults to \texttt{True}.
%\textbf{System dynamic condition $\bm{T}$, }
% how the environment transits from the current state $x_i$ to the new state $x_{i+1}$. 
% Generally, the action $N(x_i)$ taken by the agent plays a pivotal role in the state transition, but $x_{i+1}$ is not only determined by $N(x_i)$ but also affected by random factors, which necessitates the use of over-approximation~\cite{overapproximation} when describing $T$. 
\if false
\textbf{and Other condition $\bm{C}$.} In $\bm{C}$, 
extra constraints related to specified properties are encoded.
This part stands apart from the $\bm{S},\bm{T},\bm{I}$ parts usually describing the unchanging characteristics of a particular DRL system. For example, some liveness properties require no \texttt{bad} state cycle existing~\cite{mc,whiRL}; and this constraint should be considered as an extra constraint due to its exclusive association with this particular property, rather than a characteristic of the system.
We believe that distinct division in this way is beneficial for users to formulate and articulate properties.
\fi
 
%\textbf{Post-condition $\bm{Q}$} is the expected verification result under pre-condition $\bm{P}$. 
% Safety properties~\cite{MC} represent one of the paramount property types, where the agent is expected to persistently avoid undesirable actions under given pre-conditions. Safety properties guarantee that the DRL system will never transition into \textit{bad} states. The predicate $Good(N(x))$ evaluates as \texttt{True} when in \textit{good} states and vice versa. Such a property is formulated as:
% \begin{equation}
% \begin{split}
%         \forall x_0,x_1..., &\bigwedge_{i=0}(S(x_i)\wedge I(x_i)\wedge T(x_i)\wedge C(x_i)) \\
%         &\to \bigwedge_{i=0}(Good(N(x_i)))
% \end{split}
% \end{equation}

% Another type of property is liveness property~\cite{MC}, where the agent might take undesirable actions but is expected to eventually take desirable ones. Liveness properties guarantee that the DRL system will not remain persistently trapped in \textit{bad} states. Thus, verifying liveness properties involves the detection of cycles of states consistently in \textit{bad} states. $C'(x)$ denotes $C(x)$ without cycle detection, i.e., $x_i != x_\gamma$. Such a property is formulated as:

% \begin{equation}
% \begin{split}
%         \forall x_0,x_1..., &\bigwedge_{i=0}(S(x_i)\wedge I(x_i)\wedge T(x_i)\wedge C'(x_i) \\ & \wedge(\bigwedge_{\gamma=0}^{i-1} (x_i != x_\gamma))) 
%         \to \bigvee_{i=0}(Good(N(x_i)))
% \end{split}
% \end{equation}

% Robustness properties assess the stability of the agent's performance within adversarial environments, which constrains the agent to take consistent or similar actions in the presence of perturbed input values (local robustness~\cite{robness}) or input outliers (extreme value robustness~\cite{Reluplex}. $\hat{x_{0}}$ denotes the original input, and $\varepsilon$ denotes perturbation. Such a property is formulated as: 
% \begin{equation}
%         \forall x_0, I(x_0)\wedge C(x_0)\to N(x_0) \approx N(\hat{x_{0}})
% \end{equation}
% For local robustness, $I(x_0)\equiv \bigwedge_{i=0} (\hat{x_{0}^i} -\varepsilon^i \le x_0^i \le \hat{x_{0}^i} +\varepsilon^i)$; for extreme value robustness, $I(x_0)\equiv \bigwedge_{i \in D} (\hat{x_{0}^{i}} -\epsilon^i \le x_0^i \le \hat{x_{0}^{i}} +\epsilon^i) \wedge \bigwedge_{i \in R} (\hat{x_{0}^{i}} -\varepsilon^i \le x_0^i \le \hat{x_{0}^{i}} +\varepsilon^i)$, in which $D$ denotes the set of indices of the input values with outliers, while $R$ denotes the set of indices of other input values.

\subsubsection{DRLP Script.}

The DRLP verification script can be structurally divided into three segments.
The first segment initializes a series of pre-assigned variables used for the verification.  
The second segment, starting with a delimiter \texttt{@Pre}, is a set of the pre-conditions $P$ (the properties and the trained DRL system).
The third segment, starting with a delimiter \texttt{@Exp}, is a set of the post-conditions $Q$ (the expected verfication results). 
In the script, \texttt{x} denotes the input of DNN, \texttt{y} denotes the output of DNN and \texttt{k} denotes the verification depth; variables prefixed with ``\_'' are categorized as \textsl{iterable variables}. %For a more comprehensive definition of the DRLP syntax, refer to the appendix.
Fig.~\ref{DRLPExample} shows four verification scripts encoded with the properties and a trained DRL system with two state features and one continuous action.

\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{images/drlp_s.pdf}
\caption{Illustration of four verification scripts characterizing the properties on (a) safety, (b) liveness, (c) local robustness and (d) extreme value robustness.
%\yzx{Two verification scripts characterizing the properties of (a) safety, (b) liveness, and the DRL system itself; and two verification scripts characterizing the properties of 
%(c) local robustness and (d) extreme value robustness.}
} \label{DRLPExample}
\end{figure*}


\paragraph{Safety and Liveness Property.} 
% A safety property (Fig.~\ref{DRLPExample}(a)) and a liveness property (Fig.~\ref{DRLPExample}(b)) are encoded in DRLP format. $\bm{S}$: each input value is in the range $[-1, 1]$ (Line 3); $\bm{I}$: considering two situations (Line 1), each initial input value is $0$ or $1$ (Line 4); $\bm{T}$: each value of the next state increases by at most $0.5$ when the output $> 0$ (Line 5,6), and decreases by at most $0.5$ when the output $\le 0$ (Line 5,7). For the safety property, $\bm{Q}$: outputs are always not less than $-2$ (Line 11). For the liveness property, $\bm{Q}$: outputs are eventually not less than $-2$ (Line 11,12); $\bm{C}$: no state cycle (Line 8,9).

A verification script on the safety property is shown in Fig.~\ref{DRLPExample}(a).
We first detail pre-conditions (Line 3-7).
Each state feature $x$ belongs to the interval $[-1, 1]$ (Line 3).
Considering two cases that \texttt{a} equals $0$ or $1$ (Line 1), the value of each initial state feature is respectively $0$ or $1$ (Line 4).
Note that each value of the next state increases by at most $0.5$ if the action is greater than $0$ (Line 5,6), and decreases by at most $0.5$ otherwise. 
The post-condition is that the action should always be not less than $-2$ (Line 11). 
Different from the safety property, the liveness property (Fig.~\ref{DRLPExample}(b)) enforces the additional pre-conditions that no state cycle exists (Line 8,9) and the post-condition is that the action should be eventually not less than $-2$ (Line 11,12).

\paragraph{Robustness Property.} 
%A local robustness  (Fig.~\ref{DRLPExample}(c)) and an extreme value robustness property (Fig.~\ref{DRLPExample}(d)) are encoded as examples. The original input is vector $\langle 1,0\rangle$ and its corresponding output is $0$ (Line 3). For the local robustness, $\bm{I}$: considering two degrees of perturbations \texttt{x\_eps} equals $0.01$ and $0.1$ (Line 1), each initial input value is perturbed (Line 5); we expect that the output's change should be not more than $0.2$ (Line 2,11). For the extreme value robustness, $\bm{I}$: considering two degrees of outliers $10$ and $20$ (Line 1), only the first initial input value is the outlier while the second not (Line 5); $\bm{Q}$: the output's deviation is not more than $1$ (Line 2,11).
A verification script on the local robustness property is
shown in Fig. 3(c). The pre-condition is that considering two degrees of perturbations \texttt{x\_eps} (equals $0.01$ or $0.1$) respectively (Line 1), each input feature is perturbed accordingly
% on the original input $\langle 1,0\rangle$ 
(Line 5). The post-condition (Line 11) is that the output's deviation to its original output \texttt{y\_original} (equals 0) should not exceed \texttt{y\_eps} (equals $0.2$). 
Another verification script on extreme value robustness is shown in Fig. 3(d). 
The pre-condition is that considering two degrees of outliers \texttt{x\_eps} (equals $10$ or $20$) respectively (Line 1), only the first input feature is the outlier while the second is not (Line 5). The post-condition (Line 11) is that the output's deviation to its original output \texttt{y\_original} (equals 0) should not exceed \texttt{y\_eps} (equals $1$).

% the original input is vector $\langle 1,0\rangle$ and its corresponding output is $0$ (Line 3);  considering two degrees of outliers $10$ and $20$ (Line 1), only the first input feature is the outlier while the second not (Line 5); we expect that the output's change is not more than $1$ (Line 2,11).}


% \subsection{Verification Algorithm Module}

% \paragraph{BMC}
% As the verification depth $k$ increases from $1$, both the original DNN and the DRLP are unrolled or translated with depth $k$. Then, DNN verification framework is queried. The query is formulated as:

% % If no violation is found in the verification query, increase $k$ and continue verification; but if a violation is found, the property does not hold and stop verification; if always no violation is found within maximum verification depth, it means that the property stands a good chance of holding.

% \begin{equation}
% % \small
% \begin{split}
%     \forall x_0,...,x_{k-1}, &(\bigwedge_{i=0}^{k-1}{(S(x_i)\wedge C(x_i))}) \wedge I(x_0) \\
%     & \wedge(\bigwedge_{i=0}^{k-2}{T(x_i, x_{i+1})}) \rightarrow  \bigwedge_{i=0}^{k-1}{Q((N(x_i))}
% \end{split}
% \end{equation}

% \paragraph{$\bm{k}$-induction}
% The first phase of $k$-induction, the basic situation verification, is identical to the BMC process; while the second phase diverges. In the inductive hypothesis verification, the original DNN is unrolled with depth $k+1$, and DRLP is translated for indication verification with depth $k+1$ and an assumption that the property holds with depth $k$. Then, DNN verification framework is queried. The query is formulated as:
% \begin{equation}
% % \small
% \begin{split}
%     \forall x_\alpha,...,x_{\alpha+k},  &(\bigwedge_{i=\alpha}^{\alpha+k}{(S(x_i)\wedge C(x_i))}) \wedge(\bigwedge_{i=\alpha}^{\alpha+k-1} (T(x_i \\
%     & ,x_{i+1}) \wedge Q(N(x_i)))\rightarrow Q(N(x_{\alpha+k}))
% \end{split}
% \end{equation}


% \subsection{Verification \& Interpretability Extension Module}
% Leveraging our first insight, we introduce \textit{Batch Verification} Module. Furthermore, capitalizing on the relationship between verification and interpretability and leveraging our second insight, we introduce Interpreter.


% \subsection{Batch Verification} 
% A quantitative property can be verified in batches by varying the values of \yzx{input} parameters and concreting these parameters (replacing parameters with specified values), 
% \yzx{then by analyzing the parameters and corresponding results, we can determine the quantitative characteristics of qualitative properties, }
% and we name this approach \textsl{batch verification}. 
% % A single DRL verification query, i.e., one-time verification on a DNN and a DRLP with all concreted values, is executed; but
% % \textit{Concreting}
% % a qualitative \textit{abstract property} 
% % Quantifying a qualitative property remains a formidable challenge. 
% % Taking a qualitative property that the computer should decrease its data sending rate in \texttt{bad} network conditions for example, quantifying what conditions are \texttt{bad} is tricky. 
% % Therefore, instead of being mired in such quantification, a more efficient approach is to verify in \textsl{batches} through concreting (replacing parameters in templates on qualitative property) template (script including parameters without specified values) with varying values. 
% A DRLP template is a type of DRLP script characterized by the inclusion of parameters that are not concrete specific values, and a template is encoded from a quantitative property.
% % \textsl{Batch verification} returns the pairs consisting of a Boolean verification result and its corresponding parameter values, i.e., numeric verification results.
% % Therefore, properties that share the same structures while varying the values of certain parameters can be verified in batches, and we name this approach \textsl{batch verification}. 
% DRLP supports template syntax, facilitating the efficient translation of numerous concrete scripts from a single template. 
% The scripts depicted in Fig.~\ref{DRLPExample} exemplify this capability, functioning as templates where each is adaptable to two distinct cases.
% %\subsection{Breakpoints Searching}\label{asdasd}

% The input of \textsl{batch verification} is a sequence of \jiaqi{parameter values}. 
% If the adjacent two inputs lead to the reverse verification results, i.e., from \texttt{True} to \texttt{False} or vice versa, we term such \jiaqi{scripts} as \textsl{breakpoints}.
%  % We posit that these reversals hold the potential to illuminate the inherent characteristics and decision-making rules of the DRL system.
% We design Algorithm~\ref{alg:find_bps} to identify \textsl{breakpoints}, with three representative methods in the function $step$
% % Algorithm~\ref{alg:step}
% , i.e., linear stepping, binary stepping, and iterative stepping. 
% %By utilizing \textsl{breakpoints}, \rf~is capable of indicating the boundary where the properties hold or not.
% \yzx{By extracting parameter values from the identified \textsl{breakpoints} in batch verification, we can obtain a more precise quantification in terms of the training procedure that can indicate the further need for the training model.}
% \yzx{The scripts in the identified \textsl{breakpoints} correspond to the strictest properties where the model can maintain predefined safety, liveness, or robustness.}
% % The parameter value at a breakpoint represents the maximal parameter value within a template. This value corresponds to the threshold at which a model is able to sustain critical properties such as safety, liveness, or robustness
% % }
% For example, the target model should satisfy $\phi \equiv x > 0 \Rightarrow N(x) > 0$. However, identified \textsl{breakpoints} reveals that initially, the model only satisfies $\phi \equiv x > 0 \Rightarrow N(x) > -5$, and then advances to $\phi \equiv x > 0 \Rightarrow N(x) > -2$. \jiaqi{Add a sentence: I cannot see the breakpoint happens} These sequence verification results can \jiaqi{XXX}.

% % \begin{figure*}[!tb]
% %     \centering
% %     \label{alg:alg}    
% %     \includegraphics[width=\textwidth]{images/alg.pdf}
% % \end{figure*}

% \bgroup
% \setlength{\textfloatsep}{12pt plus 1.0pt minus 2.0pt}
% \setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt}
% \setlength{\intextsep}{5pt plus 1.0pt minus 2.0pt}
% \begin{figure}[t]
% \noindent\begin{minipage}[!t]{0.49\textwidth}
% \begin{algorithm}[H]
%     \scriptsize
%     \algsetup{linenosize=\tiny}
%     \caption{find\_\textit{breakpoints}}
%     \label{alg:find_bps}
    
%     \textbf{Input}: DRLP template $p$, DNN $N$, variable list $kwgs$\\
%     \textbf{Output}: A breakpoints list $bps$ \\
%     \begin{algorithmic}[1]
%         \STATE $var \gets $ pop($kwgs$)
%         \STATE $lb, \gets $ lower bound of $var$
%         \STATE $ub \gets $ upper bound of $var$
%         \STATE $prec \gets $ required precise of $var$
%         \STATE $curr\_r \gets$ \texttt{None}
%         \STATE 
%         \WHILE{\texttt{True}}   
%             \STATE $lb,ub,curr \gets$ 
%             \STATE \ \ \ \  $step(lb,ub,curr,prec,p,N,kwgs)$ 
%             \IF{$curr = \texttt{None}$  }
%             \STATE \textbf{break} 
%             \ENDIF
%             \STATE $script \gets concrete(p,var,curr)$
%             \IF{$kwgs$ is empty }
%                 \IF{verify($script$,$N$) $\neq curr\_r$}
%                     \STATE $curr\_r \gets \neg curr\_r$ 
%                     \STATE Add $script$ to $bps$
%                 \ENDIF
%             \ELSE
%                 \STATE $find\_breakpoints(drlp,N,kwgs)$
%             \ENDIF
%         \ENDWHILE
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \begin{minipage}[!t]{0.51\textwidth}
% \begin{algorithm}[H]
%     \scriptsize
%     \algsetup{linenosize=\tiny}
%     \caption*{\textbf{Function} \textit{step}}
%     \label{alg:step}
%     \textbf{Output}: $lb$, $ub$, $curr$ 
%     \\ 
%     \\
%     \begin{algorithmic}[1]
%         \STATE $curr \gets None$
%         \STATE $lb\_r \gets verify(concrete(p,var,lb,kwgs) , N)$
%         \STATE $ub\_r \gets verify(concrete(p,var,ub,kwgs) , N)$
%         \STATE
%         \IF[Linear Stepping]{$curr \leq lb$}  
%             \STATE $curr \gets curr + prec$
%         \ENDIF
%         \STATE
%         \IF[Binary Stepping]{$ub-lb > prec$}
%             \IF{$lb\_r \neq curr\_r$}
%                 \STATE $ub\gets curr$
%                 \STATE $curr \gets \frac{lb+curr}{2}$
%             \ELSIF{$ub\_r \neq curr\_r$}
%                 \STATE $lb\gets curr$
%                 \STATE $curr \gets \frac{ub+curr}{2}$
%             \ENDIF
%         \ENDIF
%         \STATE
%         \IF[Iterative Stepping]{$lb\_r = curr\_r$ }
%             \STATE $curr \gets curr \times step$
%         \ELSE
%             \STATE $ub \gets curr$
%         \ENDIF
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \end{figure}
% \egroup


\subsection{Batch Verification} 
We introduce batch verification that can feed a sequence of parameter values, a DRLP template and model into the single verifier of \rf~and further use \textsl{breakpoints} search algorithm to  obtain a set of \textsl{breakpoints} (the scripts where adjacent two inputs lead to the reverse verification results, i.e., from \texttt{True} to \texttt{False} or vice versa). 
%A quantitative property can be verified in batches by varying the values of \yzx{input} parameters and concreting these parameters (replacing parameters with specified values), 
By extracting parameter values from the identified \textsl{breakpoints}, we can obtain a more precise numeric quantification in terms of the training procedure that can indicate the further need for the training model than conventional Boolean verification results.

% By analyzing the input parameters and the output numeric results, we can determine \jiaqi{the quantitative characteristics of qualitative properties, }
% During batch verification, if the adjacent two inputs lead to the reverse verification results, i.e., from \texttt{True} to \texttt{False} or vice versa, we term such \jiaqi{scripts} as \textsl{breakpoints}.




A DRLP template is a type of DRLP script characterized by the inclusion of parameters that are not concrete specific values, and can be encoded from a qualitative property. 
% In contrast, in a normal DRLP script, all parameters are concreted with specific values, and such a script can be encoded from a quantitative property.
% DRLP supports template syntax, facilitating the efficient translation of numerous concrete scripts from a single template. 
The scripts depicted in Fig.~\ref{DRLPExample} excluded by the first segment can be viewed as templates.
By introducing iterable variables or feeding a sequence of parameter values, each template can be translated into concrete scripts with multiple cases.

Furthermore, we design Algorithm~\ref{alg:find_bps} to identify \textsl{breakpoints}, with three representative methods in the function $step$
% Algorithm~\ref{alg:step}
, i.e., linear stepping, binary stepping, and iterative stepping. 
%By utilizing \textsl{breakpoints}, \rf~is capable of indicating the boundary where the properties hold or not.
% \yzx{By extracting parameter values from the identified \textsl{breakpoints} in batch verification, we can obtain a more precise quantification in terms of the training procedure that can indicate the further need for the training model.}\delete{than Boolean verificaiton results}
\yzx{The identified \textsl{breakpoints} correspond to the strictest properties where the model can maintain predefined safety, liveness, or robustness.}
For example, the target model should satisfy the safety property $\phi \equiv x > 0 \Rightarrow N(x) > 0$. However, identified \textsl{breakpoints} reveals that initially, the strictest property that the model satisfies is formulated as $\phi \equiv x > 0 \Rightarrow N(x) > -5$, and then advances to $\phi \equiv x > 0 \Rightarrow N(x) > -2$.  These numeric verification results extracted from the parameters in the properties, specifically -5 and -2, can demonstrate that the model is progressively becoming safer, indicating the efficacy of the preceding training strategy.


% These numerical verification results, specifically -5 and -2, extracted from these properties furnish a more precise quantification of the model's progression compared to mere Boolean \texttt{False} which only indicates the need for further training.




% \begin{figure*}[!tb]
%     \centering
%     \label{alg:alg}    
%     \includegraphics[width=\textwidth]{images/alg.pdf}
% \end{figure*}

\bgroup
\setlength{\textfloatsep}{12pt plus 1.0pt minus 2.0pt}
\setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt}
\setlength{\intextsep}{5pt plus 1.0pt minus 2.0pt}
\begin{figure}[t]
\noindent\begin{minipage}[!t]{0.49\textwidth}
\begin{algorithm}[H]
    \scriptsize
    \algsetup{linenosize=\tiny}
    \caption{find\_\textit{breakpoints}}
    \label{alg:find_bps}
    
    \textbf{Input}: DRLP template $p$, DNN $N$, variable list $kwgs$\\
    \textbf{Output}: A breakpoints list $bps$ \\
    \begin{algorithmic}[1]
        \STATE $var \gets $ pop($kwgs$)
        \STATE $lb, \gets $ lower bound of $var$
        \STATE $ub \gets $ upper bound of $var$
        \STATE $prec \gets $ search precise of $var$
        \STATE $curr\_r \gets$ \texttt{None}
        \STATE 
        \WHILE{\texttt{True}}   
            \STATE $lb,ub,curr \gets$ 
            \STATE \ \ \ \  $step(lb,ub,curr,prec,p,N,kwgs)$ 
            \IF{$curr = \texttt{None}$  }
            \STATE \textbf{break} 
            \ENDIF
            \STATE $script \gets concrete(p,var,curr)$
            \IF{$kwgs$ is empty }
                \IF{verify($script$,$N$) $\neq curr\_r$}
                    \STATE $curr\_r \gets \neg curr\_r$ 
                    \STATE Add $script$ to $bps$
                \ENDIF
            \ELSE
                \STATE $find\_breakpoints(drlp,N,kwgs)$
            \ENDIF
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}[!t]{0.51\textwidth}
\begin{algorithm}[H]
    \scriptsize
    \algsetup{linenosize=\tiny}
    \caption*{\textbf{Function} \textit{step}}
    \label{alg:step}
    \textbf{Input}: lower bound $lb$, upper bound $ub$, current position $curr$, search precise $prec$, DRLP template $p$, DNN $N$, variable list $kwgs$\\
    \textbf{Output}: lower bound $lb$, upper bound $ub$, current position $curr$ 
    \begin{algorithmic}[1]
        \STATE $curr \gets None$
        \STATE $lb\_r \gets verify(concrete(p,var,lb,kwgs) , N)$
        \STATE $ub\_r \gets verify(concrete(p,var,ub,kwgs) , N)$
        \STATE
        \IF[Linear Stepping]{$curr \leq lb$}  
            \STATE $curr \gets curr + prec$
        \ENDIF
        \IF[Binary Stepping]{$ub-lb > prec$}
            \IF{$lb\_r \neq curr\_r$}
                \STATE $ub\gets curr$
                \STATE $curr \gets \frac{lb+curr}{2}$
            \ELSIF{$ub\_r \neq curr\_r$}
                \STATE $lb\gets curr$
                \STATE $curr \gets \frac{ub+curr}{2}$
            \ENDIF
        \ENDIF
        \IF[Iterative Stepping]{$lb\_r = curr\_r$ }
            \STATE $curr \gets curr \times step$
        \ELSE
            \STATE $ub \gets curr$
        \ENDIF
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
\egroup




\subsection{Interpretation}
%Answering interpretability questions is a crucial strategy for achieving \jiaqi{interpretable machine learning.} 
Answering interpretability problems can evaluate the behaviors of the trained models and provide useful insight to its underlying decision-making mechanisms.
Wildly concerned interpretability problems include decision boundary~\cite{iw26,iw43}, counterfactual explanation~\cite{iw28,iw29}, sensitivity analysis~\cite{iw27} and importance analysis~\cite{iw8}. 
Our proposition is a cohesive methodology to these problems, fundamentally reliant on the identified \textit{breakpoints}. Our methodology has the potential to address a broader spectrum of interpretability concerns.
% Our designed interpreter can answer the following interpretability questions using the identified \textit{breakpoints}.

\subsubsection{Decision Boundary.}
For a robustness property ~\cite{iw42,iw43}, the data points, which are formed by the parameters extracted from the \textsl{breakpoints}, are part of the decision boundary. This perspective inspires us to discern the specific conditions under which the DRL system satisfies given safety, liveness, and robustness properties. Additionally, in the context of safety and liveness properties, if the verification depth is confined to $k=1$, i.e., degenerating into one-shot DNN verification, the parameters extracted from the identified \textit{breakpoints} are also recognized as invariants~\cite{whiRL_2.0}, which indicates the boundary between conditions wherein the property always holds or always not. 

\textbf{Our solution:} Find \textit{breakpoints} by stepping through interested parameters; and fit the corresponding decision boundary with the data points 
consisting of parameters extracted from these \textit{breakpoints}. 

\subsubsection{Intuitiveness Examination.}
An intuitive insight of the example of sending data using the computer: the worse the network condition is, the more reasonable for the computer to decrease its sending rate. When focusing on safety and liveness properties, as the values of certain parameters in the property increase or decrease, the associated constraints will consequently become more tightened or relaxed, rendering the property either easier or harder to hold; and this idea leads us to propose the intuitiveness examination. 

\textbf{Our solution: }
Find \textit{breakpoints} by linear stepping through interested parameters; and if the count of the identified \textit{breakpoints} is either $0$ or $1$, the intuitiveness examination passes. $bps$ denotes the list of identified \textit{breakpoints}, and the answer to this question is formulated as:

\begin{equation}
    size\_of(bps) = 0 \vee size\_of(bps) = 1
\end{equation}

\subsubsection{Counterfactual Explanation.} 
Given the original input $\hat{x_0}$ and the target counterfactual output $\hat{y_0}$ such that $\hat{y_0}\not\approx N(\hat{x_0})$, the counterfactual explanation question~\cite{iw28,iw29} aims to identify the counterfactual inputs $\{x_0\}$ such that $N(x_0) \approx \hat{y_0}$. The most valuable counterfactual input $x_0$ is the one that is closest (according to vector distance) to the original input $\hat{x_0}$. Because the minimum vector distance often implies the minimum attack cost~\cite{Attack}, this counterexample can effectively highlight the system's weakness.

% \begin{equation}
% % \small
% \begin{split}
%         \forall x_0,x_1..., & \bigwedge_{i=0}((\bigwedge_{j=0}^{n-1}(\hat{x_{i}^{j}} -\varepsilon_i^j \le x_i^j \le \hat{x_{i}^{j}} +\varepsilon_i^j)) \wedge \\
%         & T(x_i)\wedge C(x_i)) 
%         \to \bigwedge_{j=0}(Q(N(x_i)))
% \end{split}
% \end{equation}

% \begin{equation}
% % \small
% \begin{split}
%         &\forall x_0,x_1...,  \bigwedge_{i=0}((\bigwedge_{j=0}^{n-1}(\hat{x_{i}^{j}} -\varepsilon_i^j \le x_i^j \le \hat{x_{i}^{j}} +\varepsilon_i^j) \wedge T(x_i)\\
%         & \wedge C'(x_i)\wedge(\bigwedge_{\gamma=0}^{i-1} (x_i != x_\gamma))) 
%         \to \bigwedge_{j=0}(Q(N(x_i)))
% \end{split}
% \end{equation}


\textbf{Our solution: } 
Find \textit{breakpoints} by stepping through possible perturbation value $\varepsilon_0^j$ of each input $x_0^j$ on the property formulated as:
\begin{equation}
% \small
         \forall x_0, \bigwedge_{j=0}^{n-1}(\hat{x_{0}^{j}} -\varepsilon_0^j \le x_0^j \le \hat{x_{0}^{j}} +\varepsilon_0^j) \Rightarrow N(x_0) \approx \hat{y_0}
\end{equation}
Here, we expand the question to encompass safety and liveness properties as well: safety, $    P
\equiv \bigwedge_{i=0}((\bigwedge_{j=0}^{n-1}(\hat{x_{i}^{j}} -\varepsilon_i^j \le x_i^j \le \hat{x_{i}^{j}} +\varepsilon_i^j)) \wedge  T \wedge I) $; liveness, $P(x) \equiv \bigwedge_{i=0}((\bigwedge_{j=0}^{n-1}(\hat{x_{i}^{j}} -\varepsilon_i^j \le x_i^j \le \hat{x_{i}^{j}} +\varepsilon_i^j) \wedge T
\wedge I \wedge(\bigwedge_{\gamma=0}^{i-1} (x_i != x_\gamma)))$. Finally, the answer is the closest one, which is formulated as:
\begin{equation}
% \small
    \arg\min_{bp\in bps} distance\_of(\hat{x}+\varepsilon,\hat{x})
\end{equation}

\subsubsection{Sensitivity Analysis.} 
Given the original input $\hat{x_0}$ and the perturbation $\varepsilon$, the sensitivity analysis question~\cite{iw27} aims to evaluate the distances between $N(x_0)$ and $N(\hat{x_0})$, where $x_0$ denotes the input whose features under discussion are subjected to the perturbation $\varepsilon$. Sensitivity analysis on all input features identifies which specific feature with a higher sensitivity analysis result has the potential to induce greater fluctuations in the output.
 

\textbf{Our solution: } 
Find \textit{breakpoints} by stepping through possible $y_0$ on the property formulated as:
\begin{equation}
         \forall x_0, \bigwedge_{j \in D} (\hat{x_{0}^{j}} -\varepsilon \le x_0^j \le \hat{x_{0}^{j}} +\varepsilon) \wedge \bigwedge_{j \in R} (\hat{x_{0}^{j}}=x_0^j) \Rightarrow N(x_0) \approx y_0
\end{equation}
where $D$ denotes the set of indices of the discussed features within the input, while $R$ denotes the set of indices of other features.
Finally, the answer is the minimum distance between $y_0$ and $N(\hat{x_0})$, i.e., sensitivity, which is formulated as:
\begin{equation}
% \small
    \min_{bp\in bps} distance\_
    of(y_0,N(\hat{x_0}))
\end{equation}


\subsubsection{Importance Analysis.}
Given the original input $\hat{x_0}$, the importance analysis question~\cite{iw8} aims to evaluate the distances between $x_0$ and $\hat{x_0}$,
where $x_0$ denotes the input whose features under discussion can be perturbed such that $N(x_0) \not\approx N(\hat{x_0})$.
The lower the distance, the more important the feature; since even a slight perturbation in the input of such a feature can induce greater fluctuations in the output. Importance analysis on all input features identifies which specific feature holds a central role in the decision-making process.

\textbf{Our solution: } 
Find \textit{breakpoints} by stepping through possible perturbation values $\{\varepsilon^j_0\}$ applied to the input features $\{x_0^j\}$ on the property formulated as:
\begin{equation}
% \small
% \begin{split}
     \forall x_0, \bigwedge_{j \in D} (\hat{x_{0}^{j}} -\varepsilon^j_0 \le x_0^j \le \hat{x_{0}^{j}} +\varepsilon^j_0) \wedge \bigwedge_{j \in R} (\hat{x_{0}^{j}}=x_0^j)  \Rightarrow N(x_0) \not \approx N(\hat{x_0})
% \end{split}
\end{equation}
where $D$ and $R$ denote the same sets in the sensitivity analysis.
Finally, the answer is the minimum distance between $\hat{x_0}+\varepsilon$ and $\hat{x_0}$, i.e., importance, which is formulated as:
\begin{equation}
% \small
    \min_{bp\in bps} distance\_of(\hat{x_0}+\varepsilon,\hat{x_0})
\end{equation}

% $



==> sections/Rtrback.tex <==


\section{The Property-Metric Gap-Based
Algorithm }
% \paragraph{Reward shaping}
% Note that the strategies of how the \texttt{reward\_api} returns final rewards must be thoughtfully crafted and can be subject to dynamic adjustments. Reintrainer offers various commonly used strategies:

% \textbf{(i)} Reduce rewards as penalties when desired properties are violated or increase rewards as incentives when desired properties hold. \textbf{(ii)} Vary the magnitude of penalties and incentives in relation to the advancement of rounds. \textbf{(iii)} Increase penalties and incentives for properties that carry greater significance in terms of being satisfied. \textbf{(iv)} Increase penalties and incentives for more stringent properties or more relaxed ones. 

% \subsection{Property-Metric Gap-Based Reward Shaping}
% Specifically, we present a novel property-metric gap-based algorithm for DRL with interpretability integrated.

The hypothesis we advocate posits that penalties are directly proportional to the magnitude of violations.
Furthermore, this proportionality extends to the deviation from current states 
% where the violations occur 
to those states where the property holds.
This deviation can be equivalently described as the distances between the boundary of the property-constrained spaces and the states where violations occur.

\subsection{Metric of a Single Property}





% The distance between 
%  indicates the gap from the current model in training to the ideal model in
% desired properties satisfaction
% We first measure a state dimension and then extend it to an n-dimensional state space

\subsubsection{Distance of States in $1$-Dimension.}
To elucidate our algorithm, we employ the Mountain Car~\cite{mountaincar} task as a case study. The task consists of a car placed stochastically at a valley's bottom, and its goal is to accelerate the car to reach the top of the right hill. The agent can take one of three discrete actions: accelerate to the left, to the right, or not accelerate. The environment states consist of two features: the car's position along the x-axis $p$, and the car's velocity $v$. 
% The agent is penalized with a reward of $-1$ for each timestep as long as it does not reach the target.
% In general, we believe that the closer the environmental state is to the boundary of the property-constrained space when a violation occurs, the lighter penalty the agent needs to face; and the farther it is, the more severe penalty should be. 

Considering the safety property $\phi_1$ of Mountain Car (then denoted by $\phi$, $\phi \equiv \langle p,v \rangle \in [\langle -0.60,0.03\rangle,\langle -0.40, 0.07\rangle]
\Rightarrow Action \neq 0$) defined in Evaluation,
if this property is violated under the conditions such as when $\langle p,v \rangle$ is
\textbf{(i)} $\langle -0.50,0.05 \rangle$, \textbf{(ii)} $\langle -0.41,0.05 \rangle$, \textbf{(iii)} $\langle -0.59,0.05 \rangle$, \textbf{(iv)} $\langle -0.50,0.07 \rangle$, the agent's action is 0.
 % The agent should be penalized, but penalties should vary depending on the magnitude of the violation in each condition. 


\paragraph{Raw distance.}
The agent in \textbf{(i)} should be penalized more severely than in \textbf{(ii)}, because the latter only needs to make a minor adjustment, i.e., reduce $p$ to $0.4$ to satisfy the property. Therefore, the distance from \textbf{(i)} to the boundary should be greater than the distance from \textbf{(ii)}.
Therefore, we define a raw distance function: given the state feature $s_i^j$ whose current observation is $\mathtt{v}$, its raw distance $dist'$ to its property-constrained space $\phi[s_i^j]$ in $1$-dimension is formulated as:

\begin{equation}
    dist'(\phi[s_i^j],\mathtt{v}) = min(|\underline{\phi}[x_i^j]-\mathtt{v}|,|\overline{\phi}[x_i^j]-\mathtt{v}|)
\end{equation}

%
\paragraph{Distance density.}

However, the raw distance measure $dist'$ is not sufficient for certain scenarios, such as when comparing \textbf{(ii)} with \textbf{(iii)}. In both cases, the value of 
$p$ is equally close to the boundary, yet the fluctuations in the output could be different for the same input feature at different values.
% How to quantify  the fluctuations is challenging.
This observation leads us to the concept of sensitivity analysis mentioned in interpretability questions, which is used to measure the potential of a feature to induce fluctuations in the output.

Given the DNN $N$ and the original input $\hat{x}_0$, when the input feature $x_0^j$ is subject to perturbation $\varepsilon$, the sensitivity of $x_0^j$ can be formulated as:

\begin{equation}
    % \begin{split}
            Sensitivity(N,\hat{x}_0, x_0^j) = 
            \max_{x_0} distance\_of(N(\hat{x}_0),N(x_0))
            % \\ min( 
            % &distance\_of(\max_{x_0}N(\hat{x}_0),N(x_0), \\
            % &distance\_of(\min_{x_0}N(\hat{x}_0),N(x_0))
    % \end{split}
\end{equation}
where $x_0\in[\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j-\varepsilon,...,\hat{x}_0^{n-1}\rangle,\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j+\varepsilon,...,\hat{x}_0^{n-1}\rangle]$.

% 高精度的sensitivity/场密度的本质是偏微分d(N(x_0))/x_0^j，可以通过直接对神经网络连续求导，或者直接连续让N(x_0+\epsilon)*\epsilon完成积分

% \begin{equation}
%     \begin{split}
%         Sensitivity&(N,\hat{x}_0,\varepsilon, x_0^j) = \\ min( 
%             &\|(\max_{x_0}N(\hat{x}_0)-N(x_0)\|, \\
%             &\|(\min_{x_0}N(\hat{x}_0)-N(x_0)\|)
%     \end{split}
% \end{equation}

Considering that perturbations need only be evaluated in one direction at the boundary, we define two types of sensitivity measures. The first is the sensitivity of the lower bound $\underline{Sens}(N,\hat{x}_0, x_0^j)$, where $x_0\in[\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j,...,\hat{x}_0^{n-1}\rangle,\langle\hat{x}_0^0,\hat{x}_0^1,$ $...,\hat{x}_0^j+ \varepsilon , ... , \hat{x}_0^{n-1}\rangle]$. The second is the sensitivity of the upper bound $\overline{Sens}\allowbreak(N,\hat{x}_0, x_0^j)$, where $x_0\in[\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j-\varepsilon,...,\hat{x}_0^{n-1}\rangle,\allowbreak\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j,...,\hat{x}_0^{n-1}\rangle]$.


% Multiplying the difference by the coefficient is as  we are in a space with density, so we take the result of sensitivity as the density function $\rho$ as:

% \begin{equation}
%     \begin{split}
%             \underline{\rho}(\underline{\phi}[x_i^j])=  \underline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j)  \\ 
%     \overline{\rho}(\overline{\phi}[x_i^j])=  \overline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j)  
%     \end{split}
% \end{equation}




% \paragraph{Boundary.}

Besides, in the comparison between scenarios \textbf{(i)} with \textbf{(iv)}, although $v$ in \textbf{(iv)} is closer to $\phi[v]$, the value of $v$ equaling $0.07$ is actually the upper bound of velocity in the Mountain Car environment (denoted by $\overline{S}[v]$). Therefore, a significant adjustment is needed in \textbf{(iv)}, i.e., reduce $v$ to $0.3$ to satisfy the property. Consequently, the distance from \textbf{(iv)} to the boundary should be greater than the distance from \textbf{(i)}.
As a result, we define the lower bound \textsl{density} function $\underline{\rho}$ of the state feature $x_i^j$ 
in the property $\phi$ and the DNN $N$
as:
\begin{align}
    \underline{\rho}(N,\phi,s_i^j)= \left\{
    \begin{array}{ll}
        +\infty &  \text{if }  \underline{\phi}[s_i^j] = \underline{S}[s_i^j] \\
        \underline{Sens}(N,\underline{\phi}[s], s_i^j) & \text{else} 
    \end{array}
    \right.
\end{align}
This function is also denoted as $\underline{\rho}(\phi,s_i^j)$ for simplicity.
Similarly, the upper bound \textsl{density} function $\overline{\rho}$ can be defined.
% \begin{align}
%     \overline{\rho}(\overline{\phi}[x_i^j])= \left\{
%     \begin{array}{ll}
%         +\infty & \text{if }  \hat{x}_0^j = \overline{\phi}[x_i^j] \\
%         \overline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j) & \text{else} 
%     \end{array}
%     \right.
% \end{align}


\paragraph{Exact middle point.}
The exact middle point, denoted as $\dot{\phi}[s_i^j]$, represents the position with the maximum distance to the boundary, and also the point where the \textsl{density} of the lower and upper boundaries switches. Accordingly, this point should be closer to the boundary that exhibits greater density. Consequently, we determine the exact middle point by calculating the midpoint of the \textsl{density}-weighted upper and lower bounds, which can be formulated as:

% The key lies in the definition of the exact middle $\dot{\phi}[x_i^j]$, which means that $\dot{\phi}[x_i^j]$ should not be simply $\overline{\phi}[x_i^j]$+$\underline{\phi}[x_i^j]$/2, because the same value change at $\overline{\phi}[x_i^j]$ and $\underline{\phi}[x_i^j]$ should have different effects. Approaching the same value from both sides does not necessarily mean walking the same distance towards the center. For example, we applied the same numeric perturbation at $\overline{\phi}[x_i^j]$ and $\underline{\phi}[x_i^j]$. If the impact on the output is greater at $\overline{\phi}[x_i^j]$, then it indicates that the actual distance traveled here is further.

% This is equivalent to being in a dense space, where the distance between two points, $dist (u, v) = 
% \int_{u}^{v} \rho(x) \, dx$, is equal to $dist (u, v)= \rho ABS | u-v |$.

\begin{equation}
    \dot{\phi}[s_i^j] = \frac{
    \underline{\rho}(\phi,s_i^j) \cdot \underline{\phi}[s_i^j] +
    \overline{\rho} (\phi,s_i^j) \cdot \overline{\phi}[s_i^j] }{
    \underline{\rho}(\phi,s_i^j) +
    \overline{\rho} (\phi,s_i^j)  }
\end{equation}


% where $\dot{\phi}[x_i^j]$ represents the exact middle and simplest idea is $\dot{\phi}[x_i^j]=(\overline{\phi}[x_i^j]+\underline{\phi}[x_i^j])/2$.


\paragraph{Normalization.}
% Our goal in calculating the distance between states in $1$-dimension is to measure the magnitude of deviation of a feature from a predefined property. Consequently, 
To facilitate the reasonable extension of distances from $1$-dimension to $n$-dimensions, we normalize the distance to fall within the range of $[0,1]$. 
Given the state feature $s_i^j$ whose current observation is $\mathtt{v}$, its distance $dist$ to its property-constrained space $\phi[s_i^j]$ in $1$-dimension is formulated as:
\begin{equation}
    dist(\phi[s_i^j],\mathtt{v}) = \left\{
    \begin{array}{ll}
        0 & \text{if } \mathtt{v} \in (-\infty,\underline{\phi}[s_i^j])  \\
        (\frac{\mathtt{v}-\underline{\phi}[s_i^j]}{\dot{\phi}[s_i^j]-\underline{\phi}[s_i^j]})^{p_1} & \text{if } \mathtt{v} \in [\underline{\phi}[s_i^j],\dot{\phi}[s_i^j])  \\
        1 & \text{if } \mathtt{v} = \dot{\phi}[s_i^j]  \\
        (\frac{\overline{\phi}[s_i^j]-\mathtt{v}}{\overline{\phi}[s_i^j]-\dot{\phi}[s_i^j]})^{p_1} & \text{if } \mathtt{v} \in (\dot{\phi}[s_i^j],\overline{\phi}[s_i^j]]  \\
        0 & \text{if } \mathtt{v} \in (\overline{\phi}[s_i^j],+\infty)
    \end{array}
    \right.
\end{equation}
where $p_1$ represents the penalty intensity coefficient. When $p_1>1$, larger distances are assigned even to slight violations; on the contrary, when $0<p_1<1$, larger distances are assigned only to severe violations.
Typically, we set $p_1$ to $1$.



% In an ideal scenario, we can calculate the density $\rho$ at every timestep; however, this calculation involves formal verification as described in the main text, which incurs significant overhead. For this reason, we typically reduce the frequency of updating the sensitivity, such as updating it at each episode, each epoch or each round, depending on the training time and effectiveness requirements.

% Since then, we have completed the definition of the distance function for the environmental state on a dimension.

\subsubsection{Distance of States in $n$-Dimension.}
While normalizing the distance of states in $1$-dimension addresses the issue of varying magnitudes of feature values, it is important to note that not all features contribute equally to the DNN's outputs.
In other words, certain important features may significantly affect the DNN's actual output, even if their $1$-dimensional distances are relatively small. 
Therefore, to account for these differences in feature importance, we employ a \textsl{density}-weighted $\ell^{p_2}$-norm. Given the state $s$ whose current observation is $\mathtt{s}$, its distance $Dist$ to the property-constrained space $\phi$ is formulated as:



\begin{equation}
    Dist(\phi,\mathtt{s})= \sqrt[p_2]{\sum[{\rho(\phi,s_i^j)\cdot(dist(\phi[s_i^j],\mathtt{s}_i^j))^{p_2}}]}/{\sum{\rho(\phi,s_i^j)}}
\end{equation}
where $p_2$ is typically set to 2; $\rho(\phi,s_i^j)$ is equal to $\underline{\rho}(\phi,s_i^j)$ when $\mathtt{s}_i^j<\dot{\phi}[s_i^j]$, otherwise, it equals $\overline{\rho}(\phi,s_i^j)$.
% To eliminate magnitude differences between different properties, we also normalize this distance.

% \| \langle dist(\phi[x_0^0],x_0^0),...,dist(\phi[x_{n-1}^{m-1}],x_{k-1}^{n-1})\rangle\|_l    


\subsubsection{Distance of Actions in $1$-Dimension.}
Similarly, when an action is taken near the property-constrained space's boundary, it suggests that the magnitude of the violation is minor, and the penalty should be also slight; whereas further from the boundary, the penalty should be severe. Therefore, the penalty could be likewise proportional to the distance from the action to the property-constrained space's boundary. For simplicity, a fixed value is sufficient for discrete actions.

\subsubsection{Metric of Violation or Satisfaction.}
Given the observed environmental state $\mathtt{s}$ and the action taken $\mathtt{a}$, we measure the violation($-$) or satisfaction($+$) when the property $\phi$ is violated or satisfied, which is formulated as:

% \begin{equation}
%     Diff(\phi,x,a)=-Dist (\phi,x)\times dist (\phi[a],a)
% \end{equation}
% Likewise, for incentives when a predefined property $\phi$ is satisfied with environmental states $x$ and an action taken $a$, we measure the satisfaction as:
\begin{equation}
    Diff(\phi,\mathtt{s},\mathtt{a})=\pm Dist (\phi,\mathtt{s})\times dist (\phi[a],\mathtt{a})
\end{equation}

\subsection{Metric of Gap}
We introduce the concept of \textsl{gap} to quantitatively measure the divergence between the anticipated parameter specified in the predefined property and the actual numeric results extracted from identified \textsl{breakpoints}. 

Considering the multiple features typically in the input, the computational complexity of finding \textsl{breakpoints} is relatively high. Therefore, we confine the \textsl{gap} measurement to just one parameter $z$ in a single input feature or the action.

% \begin{definition}
% For a set of constraints $P$ which constaint a space $V$, let $\Grave{P}$ which constaint a space $W$ be its \textit{relaxation}, i.e, $\Grave{P}\subseteq P$ where $V\subseteq W.$
% \end{definition}

\begin{definition}
Given the property $ \phi \equiv P\Rightarrow Q$, a \textit{relaxation} of $\phi$ is denoted by $\Grave{\phi}\equiv \Grave{P} \Rightarrow \Grave{Q}$ , where $\Grave{P}\subseteq P, \Grave{Q}\supseteq Q$.
% ; in contrast,  let $\Acute{\phi}\equiv \Acute{P} \Rightarrow \Acute{Q}$ be its \textit{tightening}, where $\Acute{P}\supseteq P, \Acute{Q}\subseteq Q$.
\end{definition}

In this context, we find \textit{breakpoints} by stepping through $z$ within the domain of $\Grave{\phi}$ on DNN $N$. Subsequently, $bps$ denotes the list of corresponding properties associated with identified \textsl{breakpoints}, and the \textsl{gap} function is formulated as:
\begin{equation}
g(\phi,N)=\min_{\Grave{\phi}\in bps} |\phi[z]-\Grave{\phi}[z]|
\end{equation}


We posit the \textit{gap} metric bears a conceptual resemblance to the learning rate in the context of property learning. Consequently, as the agent inches closer to satisfying the predefined properties, the learning rate of these properties should correspondingly diminish. To enact this adaptive learning strategy, we similarly introduce a learning rate schedule function $Lr$, which adjusts the learning rate for property learning based on the \textit{gap} value, in line with conventional practices in RL. This yields the subsequent relation:

\begin{equation}
    \Tilde{Diff}(\phi,\mathtt{s},\mathtt{a}) = Lr(g(\phi,N))\times Diff(\phi,\mathtt{s},\mathtt{a})
\end{equation}

% Another approach is to build a decision tree based on predefined properties, with constraints of a property starting from the root node and ending at a leaf node. We believe that the deeper the leaf node, the more relaxed the property. By arranging all properties according to their depth, a sequence of properties ranging from relaxed to stringent can be established, and their weights can be chosen in ascending or descending order.

\subsection{Weights for Multiple Properties}
If multiple properties are simultaneously required to be satisfied, a weight $w \in [0,1]$ can be assigned to each property. The weights can be assigned manually based on the importance or based on the preference of each property, with higher weights given to properties more likely to be satisfied. 
% Another approach is to build a decision tree based on predefined properties, with constraints of a property starting from the root node and ending at a leaf node. We believe that the deeper the leaf node, the more relaxed the property. By arranging all properties according to their depth, a sequence of properties ranging from relaxed to stringent can be established, and their weights can be chosen in ascending or descending order.
We use factor $\beta$ to scale the effect of $\Tilde{Diff}$ as a whole, and we find during the evaluation that when intermediate reward $F_t$ and $r_t$ are at the same order of magnitude, our approach works well. 
The intermediate reward function is formulated as:
\begin{equation}
    F_t = \beta\sum{w_i \Tilde{Diff}(\phi_i,\mathtt{s},\mathtt{a})}
\end{equation}


\subsection{Traceback}
For properties that span multiple steps, including multi-step safety and liveness, it is imperative to trace back to adjust the reward trajectories in the buffer before policy optimization. For instance, once a multi-step safety property is violated at a particular step, this implies increasing unsafety in the preceding trajectory, necessitating the imposition of penalties. We calculate the traced intermediate reward $\Tilde{F}_{t}$ backward from the last trajectory in the buffer with a discount factor $\lambda\in[0,1)$ as:

\begin{equation}
    \Tilde{F}_{t} = F_t + \lambda \Tilde{F}_{t+1}
\end{equation}

The final shaped reward given to the agent $\Tilde{r}_t$ is formulated as:
\begin{equation}
    \Tilde{r}_t = r_t + \Tilde{F}_{t}
\end{equation}

==> supsec/Reward.tex <==
\section{Property-Metric-Based Reward Shaping}
The primary objective for the majority of DRL tasks is to achieve their control target as quickly as possible, i.e., to maximize the cumulative reward. Additionally,  we aim to guarantee that the final models satisfy predefined properties, thereby ensuring their safety and reliability. To achieve these two goals, specifically, we present a novel property-metric-based reward shaping approach for DRL.

\subsection{Motivation}
We initiate our discussion on the condition when a property is violated during training, and a very intuitive idea is to reduce the reward as a penalty. Indeed, we hold the perspective that applying a uniform level of penalties might be deemed unreasonable. In simple terms, for a single property, even if it is violated, the extent of the violation varies, and the penalties should be more severe for more serious violations. For two properties, if one is more relaxed and relatively easier to satisfy but is violated, the penalties should be more severe than the other when violations occur; alternatively, if one carries greater significance or is preferred to satisfy, then when this property is violated, the agent should also be penalized more severely.

Therefore, how to shape reward is divided into two sub-problems: 
\begin{itemize}
    \item For a single property, measure the degree of violation or satisfaction when the property is violated or satisfied.
    \item For multiple properties, measure or determine the weights assigned to each property.
\end{itemize}

In summary, comprehensive measurements of property satisfaction or violation during training, along with thorough measurements of the properties themselves and the relationships between them, result in more effective reward shaping.


\subsection{Metric of a Single Property}
We here introduce an innovative approach that measures and quantifies the degree of property violation or satisfaction during training. Furthermore, we integrate the Sensitivity Analysis in the interpretability questions of DRL to enhance the accuracy of this measurement.

We maintain the idea that penalties are directly proportional to the degree of violations, and the degree of violations is directly proportional to the distances from current states to the states of not violating the property, which is equivalent to the \textit{distances} between the boundary of the property-constrained space and the environmental state when violations occur. 



% The distance between 
%  indicates the gap from the current model in training to the ideal model in
% desired properties satisfaction
% We first measure a state dimension and then extend it to an n-dimensional state space

\subsubsection{Distance of States in $1$-Dimension}

% In general, we believe that the closer the environmental state is to the boundary of the property-constrained space when a violation occurs, the lighter penalty the agent needs to face; and the farther it is, the more severe penalty should be. 
Taking the safety property Prop 1 (then denoted by $\phi_1$) defined for evaluation in the Mountain Car task as an example,
%\equiv p \in [-0.40, -0.60] \wedge v \in [0.03,0.07] \to Action \neq 0$%
if this property is violated, such as in the conditions when $\langle p,v \rangle$ is
\textbf{(i)} $\langle -0.50,0.05 \rangle$, \textbf{(ii)} $\langle -0.41,0.05 \rangle$,\textbf{(iii)} $\langle -0.59,0.05 \rangle$, \textbf{(iv)} $\langle -0.50,0.07 \rangle$, the agent takes an action to accelerate to the left.
 % The agent should be penalized, but penalties should vary depending on the degree of the violation in each condition. 


\paragraph{Raw distance.}

The agent in \textbf{(i)} should be penalized more severely than in \textbf{(ii)}, because the latter only needs to make a slight change, i.e., reduce $p$ to $0.4$ to satisfy the property. Therefore, the distance from \textbf{(i)} should be greater than the distance from \textbf{(ii)} to the boundary.

To address the constraint mentioned above, we define a raw distance function: for a certain feature $x_i^j$ of the environmental state whose current observation is $\mathtt{v}$, its raw distance $dist'(\phi[x_i^j],\mathtt{v})$ to its property-constrained space's boundary $\phi[x_i^j]$ in $1$-dimension is formulated as:
\begin{equation}
    dist'(\phi[x_i^j],\mathtt{v}) = min(|\mathtt{v}-\underline{\phi}[x_i^j]|,|\mathtt{v}-\overline{\phi}[x_i^j]|)
\end{equation}


%
\paragraph{Distance density.}

However, such $dist'$ cannot meet the constraint from the following scenario:

When comparing \textbf{(ii)} with \textbf{(iii)}, although $p$ in both conditions is equally close to the boundary, the fluctuations in the output should be different for the same input feature at different values. How to quantify  the fluctuations is challenging. We come up with the Sensitivity Analysis mentioned in interpretability questions,  which is used to measure the potential to induce fluctuations in the output.


% Property  $\phi_1 \equiv p \in [-0.4, -0.6] \wedge v \in [0.03,0.07] \to Action \neq 0$ is significantly more difficult to be satisfied than Property  $\phi_1' \equiv p \in [-0.45, -0.55] \wedge v \in [0.03,0.07] \to Action \neq 0$, because the latter is a necessary condition for the former. 

% 12


%23


%14


% The above two scenarios emphasize that the normalized difference, as defined in $dist'$, cannot accurately represent the actual distance.


% We came up with the importance/sensitivity mentioned in interpretability,

For a DNN $N$, when a input feature $x_0^j$ is subject to perturbation $\varepsilon$ for a given original input $\hat{x}_0$, its sensitivity can be formulated as:

\begin{equation}
    \begin{split}
            Sensitivity&(N,\hat{x}_0,\varepsilon, x_0^j) = \\
            \max_{x_0} &\  distance\_of(N(\hat{x}_0),N(x_0))
            % \\ min( 
            % &distance\_of(\max_{x_0}N(\hat{x}_0),N(x_0), \\
            % &distance\_of(\min_{x_0}N(\hat{x}_0),N(x_0))
    \end{split}
\end{equation}
where $x_0\in\langle[\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j-\varepsilon,...,\hat{x}_0^{n-1}\rangle,\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j+\varepsilon,...,\hat{x}_0^{n-1}\rangle]$.

% 高精度的sensitivity/场密度的本质是偏微分d(N(x_0))/x_0^j，可以通过直接对神经网络连续求导，或者直接连续让N(x_0+\epsilon)*\epsilon完成积分

% \begin{equation}
%     \begin{split}
%         Sensitivity&(N,\hat{x}_0,\varepsilon, x_0^j) = \\ min( 
%             &\|(\max_{x_0}N(\hat{x}_0)-N(x_0)\|, \\
%             &\|(\min_{x_0}N(\hat{x}_0)-N(x_0)\|)
%     \end{split}
% \end{equation}

Since only perturbations in one direction need to be considered on the boundary, we design sensitivity of the lower bound $\underline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j)$, where $x_0\in\langle[\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j,...,\hat{x}_0^{n-1}\rangle,\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j+ \varepsilon , ... , \hat{x}_0^{n-1}\rangle]$; and sensitivity of upper bound $\overline{Sens}\allowbreak(N,\hat{x}_0,\varepsilon, x_0^j)$, where $x_0\in\langle[\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j-\varepsilon,...,\hat{x}_0^{n-1}\rangle,\allowbreak\langle\hat{x}_0^0,\hat{x}_0^1,...,\hat{x}_0^j,...,\hat{x}_0^{n-1}\rangle]$.


Multiplying the difference by the coefficient is as  we are in a space with density, so we take the result of sensitivity as the density function $\rho$ as:

\begin{equation}
    \begin{split}
            \underline{\rho}(\underline{\phi}[x_i^j])=  \underline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j)  \\ 
    \overline{\rho}(\overline{\phi}[x_i^j])=  \overline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j)  
    \end{split}
\end{equation}


The distance function is modified as:

\begin{equation}
\begin{split}
        dist''(\phi[x_i^j],\mathtt{v}) = min(&\underline{\rho}(\underline{\phi}[x_i^j])\cdot|\mathtt{v}-\underline{\phi}[x_i^j]|, \\
        &\overline{\rho}(\overline{\phi}[x_i^j])\cdot|\mathtt{v}-\overline{\phi}[x_i^j]|)
\end{split}
\end{equation}



\paragraph{Exact Middle.}


The exact middle, denoted as $\dot{\phi}[x_i^j]$, is the point with the maximum distance to the boundary and also the point where the density of the lower and upper boundaries switches. Moreover, the midpoint should be closer to the boundary with greater density. Consequently, we place the exact middle according to the midpoint of the density-weighted upper and lower bounds, as follows:

% The key lies in the definition of the exact middle $\dot{\phi}[x_i^j]$, which means that $\dot{\phi}[x_i^j]$ should not be simply $\overline{\phi}[x_i^j]$+$\underline{\phi}[x_i^j]$/2, because the same value change at $\overline{\phi}[x_i^j]$ and $\underline{\phi}[x_i^j]$ should have different effects. Approaching the same value from both sides does not necessarily mean walking the same distance towards the center. For example, we applied the same numerical perturbation at $\overline{\phi}[x_i^j]$ and $\underline{\phi}[x_i^j]$. If the impact on the output is greater at $\overline{\phi}[x_i^j]$, then it indicates that the actual distance traveled here is further.

% This is equivalent to being in a dense space, where the distance between two points, $dist (u, v) = 
% \int_{u}^{v} \rho(x) \, dx$, is equal to $dist (u, v)= \rho ABS | u-v |$.


\begin{equation}
    \dot{\phi}[x_i^j] = \frac{
    \underline{\rho}(\underline{\phi}[x_i^j]) \cdot \underline{\phi}[x_i^j] +
    \overline{\rho} (\overline{\phi}[x_i^j]) \cdot \overline{\phi}[x_i^j] }{
    \underline{\rho}(\underline{\phi}[x_i^j]) +
    \overline{\rho}(\overline{\phi}[x_i^j]) }
\end{equation}


% where $\dot{\phi}[x_i^j]$ represents the exact middle and simplest idea is $\dot{\phi}[x_i^j]=(\overline{\phi}[x_i^j]+\underline{\phi}[x_i^j])/2$.

\paragraph{Boundary.}

When comparing \textbf{(i)} with \textbf{(iv)}, although $v$ in \textbf{(iv)} is closer to $\phi_1[v_i]$, $v=0.07$ is actually the upper bound of velocity in the Mountain Car environment, so the latter indeed needs to make a significant change, i.e., reduce $v$ to $0.3$ to satisfy the property. Consequently, the distance from \textbf{(iv)} should be greater than the distance from \textbf{(i)} to the boundary.

Therefore, we modify the density function $\rho$ as:

\begin{align}
    \underline{\rho}(\underline{\phi}[x_i^j])= \left\{
    \begin{array}{ll}
        +\infty &  \text{if }  \hat{x}_0^j = \underline{\phi}[x_i^j] \\
        \underline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j) & \text{else} 
    \end{array}
    \right.
\end{align}

\begin{align}
    \overline{\rho}(\overline{\phi}[x_i^j])= \left\{
    \begin{array}{ll}
        +\infty & \text{if }  \hat{x}_0^j = \overline{\phi}[x_i^j] \\
        \overline{Sens}(N,\hat{x}_0,\varepsilon, x_0^j) & \text{else} 
    \end{array}
    \right.
\end{align}

\paragraph{Normalization.}
Our goal in calculating the distance between states in $1$-dimension is to measure the degree of deviation of a feature from a predefined property. Consequently, we normalize the distance to the range of $[0,1]$ to facilitate the reasonable extension of distances from one dimension to $n$-dimensions. The distance is defined as follows:


\begin{equation}
    dist(\phi[x_i^j],\mathtt{v}) = \left\{
    \begin{array}{ll}
        0 & \text{if } \mathtt{v} \in (-\infty,\underline{\phi}[x_i^j])  \\
        (\frac{\mathtt{v}-\underline{\phi}[x_i^j]}{\dot{\phi}[x_i^j]-\underline{\phi}[x_i^j]})^{p_1} & \text{if } \mathtt{v} \in [\underline{\phi}[x_i^j],\dot{\phi}[x_i^j])  \\
        1 & \text{if } \mathtt{v} = \dot{\phi}[x_i^j]  \\
        (\frac{\overline{\phi}[x_i^j]-\mathtt{v}}{\overline{\phi}[x_i^j]-\dot{\phi}[x_i^j]})^{p_1} & \text{if } \mathtt{v} \in (\dot{\phi}[x_i^j],\overline{\phi}[x_i^j]]  \\
        0 & \text{if } \mathtt{v} \in (\overline{\phi}[x_i^j],+\infty)
    \end{array}
    \right.
\end{equation}
where $p_1$ represents the \textit{intensity coefficient}. A value of $p_1>1$ leads to larger distances even for slight violations, indicating more severe penalty intensity; on the contrary, a value of $0<p_1<1$ results in larger distances only for severe violations, indicating more slight penalty intensity. Typically, we set $p_1=1$.



In an ideal scenario, we can calculate the density $\rho$ at every timestep; however, this calculation involves formal verification as described in the main text, which incurs significant overhead. For this reason, we typically reduce the frequency of updating the sensitivity, such as updating it at each episode, each epoch or each round, depending on the training time and effectiveness requirements.

% Since then, we have completed the definition of the distance function for the environmental state on a dimension.

\subsubsection{Distance of States in $n$-Dimension}
We normalize the distance of states in $1$-dimension, which eliminates the differences in distance calculation due to varying feature values' magnitudes. However, this does notimply that each feature contributes equally to the neural network's output.In other words, unimportant features may not significantly affect the neural network's actual output, even if their one-dimensional distance is large. Therefore, in order to reflect the differences in the importance of various features, we employ a density-weighted $\ell^{p_2}$-norm to calculate the distance. The distance of states $x$ to a property $\phi$ is formulated as::

\begin{equation}
\begin{split}
    Dist(\phi,x)= \frac{\sqrt[p_2]{\sum{\rho(\phi[x_i^j])(dist(\phi[x_i^j],x_i^j))^{p_2}}}}{\sum{\rho(\phi[x_i^j])}}
\end{split}
\end{equation}
where $p_2$ is typically set to 2. To eliminate magnitude differences between different properties, we also normalize this distance.

% \| \langle dist(\phi[x_0^0],x_0^0),...,dist(\phi[x_{n-1}^{m-1}],x_{k-1}^{n-1})\rangle\|_l    


\subsubsection{Distance of actions in $n$-Dimension}
Similarly, an action taken near the boundary of the property-constrained space indicates that the degree of violation is not severe, and the penalty the agent faces should also be slight; whereas further from the boundary, the penalty should be server. It is our view that the penalty is likewise proportional to the \textit{distance} from the boundary of the property-constrained space to the action. For simplicity, if the action space is discrete, a fixed value is sufficient.

\subsubsection{Metric of Violation or Satisfaction for a Single Property}
To calculate the penalty when a predefined property $\phi$ is violated with environmental states $x$ and an action taken $a$, we measure the violation using the following formulation:

\begin{equation}
    Diff(\phi,x,a)=-Dist (\phi,x)\times Dist (a)
\end{equation}
Likewise, for incentives when a predefined property $\phi$ is satisfied with environmental states $x$ and an action taken $a$, we measure the satisfaction using the following formulation:
\begin{equation}
    Diff(\phi,x,a)=+Dist (\phi,x)\times Dist (a)
\end{equation}

\subsection{Metric of Weights for Multiple Properties}
Due to the requirement to satisfy multiple properties simultaneously, a weight $\beta \in [0,1]$ can be assigned to each property. The weights can be assigned manually based on the importance or based on preference of each property, with higher weights given to properties that are more like to be satisfied. Another approach is to build a decision tree based on predefined properties, with constraints of a property starting from the root node and ending at a leaf node. We believe that the deeper the leaf node, the more relaxed the property. By arranging all properties according to their depth, a sequence of properties ranging from relaxed to stringent can be established, and their weights can be chosen in ascending or descending order.

\subsection{Metric Integration}
We use factor $\alpha$ to scale the effect of $Diff$ as a whole, and we find during the evaluation that when intermediate reward $F(r_t)$ and $r_t$ are at the same order of magnitude, our approach works well. The intermediate reward function is formulated as:
\begin{equation}
    F(s_t) = \alpha\sum{\beta_i Diff(\phi_i)}
\end{equation}
The final shaped reward given to the agent $\tilde{r}_t$ is formulated as:
\begin{equation}
    \Tilde{r}_t = r_t + F(s_t)
\end{equation}




==> supsec/SSEva.tex <==
\section{Reintrainer Evaluation}
\subsection{Benchmarks}
We evaluate the effectiveness of Reintrainer on several commonly used benchmarks from Gym~\cite{gym}in DRL, i.e., Mountain Car, Pendulum and Cartpole. For each benchmark, we train three DRL systems using the corresponding vanilla DRL approach, related state-of-the-art work Trainify~\cite{trainify} and our Reintrainer, respectively. 

Mountain Car (MC)~\cite{mountaincar} task consists of a car placed stochastically at the bottom of a sinusoidal valley, and its goal is to strategically accelerate the car to reach the goal state on top of the right hill. The agent can take one of three discrete actions: accelerate to the left, not accelerate, or accelerate to the right. The environment states consist of two features: the position of the car along the x-axis $p$, and the velocity of the car $v$. The agent is penalized with a reward of $-1$ for each timestep as long as it does not reach the target, the top of the right hill.

Cartpole (CP)~\cite{cartpole} task consists of a pole attached by an un-actuated joint to a cart, which moves along a frictionless track, and its goal is to balance the pole.
The agent can take one of two discrete actions: push the cart to the left, or push the cart to the right.
The environment states consist of four features: cart position $p$, 	
cart velocity $v$, pole angle $\theta$, and pole angle velocity $\omega$. The agent is allotted with a reward of $+1$ for each timestep as long as it makes $\theta$ not exceed the threshold.

Pendulum (PD) task consists of a pendulum attached at one end to a fixed point while the other end is free and starts in a random position, and its goal is to apply torque on the free end to swing it into an upright position. 
The agent can take one continuous action: torque applied to the free end of the pendulum.
The environment states consist of three features: the free end's position along the x-axis $x$, position along the y-axis $y$, and angular velocity $\omega$. The agent is penalized with a reward of not more than $0$ for each timestep varying with position, angular velocity of the pendulum, and torque applied.

\subsection{Experimental and Evaluation Settings}
We adopt the same training configurations for each task respectively, including neural network architectures, DRL algorithms and their all hyper-parameters.
For the training process, we record the total training time and timesteps in our approach, in Trainify and in the vanilla DRL algorithms to compare the training efficiency.  We also record the number of occurrences and violations of predefined properties.

For the training result, we choose two metrics, including the satisfaction of predefined properties and cumulative reward, to evaluate and compare the reliability and performance of the final models trained for the same task. 

\subsection{Training Process Comparison}
\input{tab/Reintrainer/Properties.tex}
\input{tab/Reintrainer/TrainProcess.tex}
\input{tab/Reintrainer/TPS.tex}

For tasks MC and CP with discrete actions, we employ the DQN algorithm~\cite{dqn}. For task PD, with continuous actions, we employ the DDPG algorithm~\cite{ddpg}. During the training process, all hyperparameters for these vanilla algorithms have already been finely tuned to achieve their optimal performance. Additionally, Reintrainer directly employs these hyperparameters, which are consistent with the vanilla algorithms, while still guaranteeing the predefined properties to be satisfied. Regarding Trainify, we train two specific types: Trainify\#1 indicates that training employs the hyperparameters from its original work, while Trainify\#2 indicates that training employs the same hyperparameters as the vanilla algorithms.

For each task, we predefine certain properties related to their safety.
% and liveness.
For example, we define a safety property  Prop 1, which specifies that the car should not accelerate to the left when it is moving to the right at high speed at the bottom of the valley. Failure to meet this safety requirement can prevent the car from reaching the target on the right hilltop. We encode these properties in DRLP format, and Reintrainer is capable of translating them into reward shaping strategies at runtime. All predefined properties, along with their types, conditions, and meanings, are presented in Table~\ref{tab:train_prop}.

Efficiency is crucial in the training process. Therefore, we track both the total training time and the number of timesteps spent to obtain high-performing models through multiple training runs, as shown in Table~\ref{tab:train_proc}. It is undeniable that the vanilla algorithms have an advantage in total training time, while our approach takes more time due to the inclusion of formal verification and DRL interpretation in our reward generation strategy. However, we firmly believe that this time investment is worthwhile as it significantly enhances the reliability and verifiability of the models. The verification method of Trainify treats the neural network as a black box, providing it with an efficiency advantage. Speed improvements of Reintrainer can be achieved by parallelizing the generation of training and reward shaping strategies or by reducing their precision and update frequency.

Nevertheless, our approach holds a significant advantage over Trainify in terms of timesteps. This aligns with our approach's capability to provide precise feedback on reward shaping. It suggests that if the agent runs in an environment with high action costs, our method will still offer advantages in terms of efficiency.

% Due to the potential damage to the system caused by violations during the training process in some systems, 
We also track the number of violation occurrences. In conditions where violations occur frequently, such as in Prop 1, our approach demonstrates advantages in reducing violations. However, in environments where there are few or no violations, such as in Prop 2, Reintrainer may actively generate a smaller number of counterexamples for the agents to learn. Prop 3 is aimed to guide the agent to try to make the pendulum more upright, so more violations occurring during the training process of Reintrainer to promote the final model's performance are acceptable.

% Reintrainer




\subsection{Final Model Comparison}
We compare the cumulative rewards and the satisfaction of predefined properties for the final models obtained through our approach, Trainify, and vanilla algorithms.

\subsubsection{Cumulative Reward}
\input{tab/Reintrainer/AccReward.tex}
\input{tab/Reintrainer/AC.tex}

We evaluate the final models in Gym environments of each task for 100 episodes in a standard Gym environment. We record the cumulative rewards for each episode and then calculated their average and standard deviation, as shown in Table~\ref{tab:train_ans}. The cumulative reward is an important metric to evaluate a trained model’s performance because to maximize it is the learning objective, and a larger cumulative reward reflects better performance. The results demonstrate that our approach performs at a similar level to the vanilla algorithms, and significantly outperforms both types of Trainify in all cases.

\subsubsection{Verification}
We also formally verify the predefined properties on these final models. The results presented in Table~\ref{tab:train_ans} show that the vanilla algorithms do not guarantee these properties to be satisfied, while in some cases the property is also satisfied.
% The final models trained by Trainify only satisfy Prop 2, which we believe is related to the limitations of Trainify's approach, which only subdivides the abstract state space. Trainify performs well in terms of properties of reachability, i.e., the agent can reach specific environmental states, as Prop 2.
The final models trained by Trainify do not satisfy these properties, which we believe is related to the limitations of Trainify's approach, which only subdivides the abstract state space. Trainify performs well in terms of properties of reachability, i.e., the agent can reach specific environmental states. Although we have modified Trainify to include action detection, its approach fundamentally does not guide agents to avoid taking unexpected actions, which is typically required for safety. 

However, models trained by our approach can satisfy all predefined properties. It is worth noting that there are property violations during training in Reinfier, but the verification results showed none. This discrepancy is related to the probability that agents explore during training.


\subsection{Conclusion}
A significant advantage of Reintrainer is its complete decoupling from training algorithms and model structures, making it adaptable to any reinforcement learning environment and algorithm. In contrast, Trainify resizes the input layer of the neural network, requiring a specialized data structure to map the environment state to the resized input layer, potentially hindering the  deployment of models. However, models trained using our approach remain entirely compatible with vanilla algorithms.

Furthermore, the evaluation results of the final models indicate that compared to the vanilla algorithms, our approach guarantees property satisfaction without incurring performance penalties; compared to Trainify, our approach also demonstrates superior performance,  satisfaction guarantee of more types of properties and advantages in terms of training timesteps.




==> supsec/SupImpact.tex <==
\section{Impact Statement}\label{Appx:Impact}
The potential positive societal impacts of this paper lie in providing verifiable and interpretable safety guarantees for DRL systems. This could lead to an increasing number of DRL designers developing and designing systems based on this research, resulting in safer and more efficient systems and advancing the field's applications.
However, the potential negative societal impacts of this paper might also result in over-reliance on and excessive trust in the verification and interpretation results. Unknown issues may exist that could lead to erroneous outcomes, necessitating the use of multiple methods and approaches for thorough verification.
% However, the potential negative societal impacts of this paper might also result in over-reliance on and excessive trust in the verification and interpretation results. Unknown issues may exist that could lead to erroneous outcomes, necessitating the use of multiple methods and approaches for thorough verification.

==> tab/Reintrainer/AC.tex <==

\setlength{\extrarowheight}{2pt} 
\begin{table*}[!t]
    \centering
    \begin{tabularx}{\textwidth}{p{1.6cm}|p{2.8cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}}
    \hline
     \multicolumn{2}{l|}{\textbf{Task}} &  \multicolumn{2}{c|}{\textbf{B1}} & \multicolumn{2}{c|}{\textbf{B2}} & \multicolumn{2}{c}{\textbf{Tora}}
     \\ \hline
     \multicolumn{2}{l|}{ID} & Prop 4 & Prop 5 & Prop 6 & Prop 7 & Prop 8 & Prop 8
     \\ \hline 

     \multirow{2}{*}{\shortstack[c]{Network}} 
         & Activation Function
         & Tanh
         & Tanh
         & Tanh
         & Tanh
         & Tanh
         & Tanh
     \\ \cline{2-8}
         & Size
         & $2\times 20$
         & $2\times 20$ 
         & $2\times 100$ 
         & $2\times 100$ 
         & $3\times 100$ 
         & $3\times 200$ 
     \\ \hline

     
     \multirow{6}{*}{\shortstack[c]{Cumulative \\ Reward}} 
         & Reintrainer
         & $\bm{-119.14}$ \newline $ \bm{\pm} \phantom{1|1}\bm{0.99}$
         & $\bm{-000.00}$ \newline $ \bm{\pm} \phantom{1|1}\bm{0.00}$
         & $\bm{-20.77}$ \newline $ \bm{\pm} \phantom{1|1}\bm{0.95}$
         & $\bm{-000.00}$ \newline $ \bm{\pm} \phantom{1|1}\bm{0.00}$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
     \\ \cline{2-8}
         & Trainify\#1
         & $-122.00$ \newline $ \pm \phantom{11}0.00$
         & $-000.00$ \newline $ \pm \phantom{11}0.00$
         & $-23.72$ \newline $ \pm \phantom{11}0.69$
         & $-000.00$ \newline $ \pm \phantom{11}0.00$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
     \\ \cline{2-8}
         & Vanilla
         & $-120.00$ \newline $ \pm \phantom{11}0.00$
         & $-000.00$ \newline $ \pm \phantom{11}0.00$
         & $-20.85$ \newline $ \pm \phantom{11}0.88$
         & $-000.00$ \newline $ \pm \phantom{11}0.00$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
         & $\phantom{+0}\bm{50.00}$ \newline $ \bm{\pm} \phantom{11}\bm{0.00}$
     \\ \hline

      \multirow{3}{*}{\shortstack[c]{Verification \\ Result}} 
         & Reintrainer
         & $\textbf{\texttt{True}}$
         & $\textbf{M}$
         & $\textbf{\texttt{True}}$
         & $\textbf{M}$
         & $\textbf{\texttt{True}}$
         & $\textbf{\texttt{True}}$
     \\ \cline{2-8}
         & Trainify\#1
         & $\textbf{\texttt{True}}$
         & $\textbf{M}$
         & $\texttt{False}$
         & $\textbf{M}$
         & $\texttt{False}$
         & $\texttt{False}$
     \\ \cline{2-8}
         & Vanilla
         & $\textbf{\texttt{True}}$
         & $\textbf{M}$
         & $\textbf{\texttt{True}}$
         & $\textbf{M}$
         & $\texttt{False}$
         & $\texttt{False}$
     \\ \hline


    \end{tabularx}


    \caption{Comparison of the final models trained by Reintrainer, Trainify and vanilla algorithms.}
    \label{tab:train_ans}
\end{table*}



==> tab/Reintrainer/TPS.tex <==

% Reintrainer
% Trainify#1
% Trainify#2
% Vanilla    /home/kurayuri/Reinfier/train_tmp/mc/mc_base#1

% RF /home/kurayuri/Reinfier/train_tmp/mc/mc_rf#2
% Tf#2 p1
% tf#1 p1_#1

\setlength{\extrarowheight}{2pt} 
\begin{table*}[!t]
    \centering
    \begin{tabularx}{\textwidth}{p{1.6cm}|p{2.8cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}|p{1.65cm}}
    \hline
     \multicolumn{2}{l|}{\textbf{Task}} &  \multicolumn{2}{c|}{\textbf{B1}} & \multicolumn{2}{c|}{\textbf{B2}} & \multicolumn{2}{c}{\textbf{Tora}}
     \\ \hline
     \multicolumn{2}{l|}{Algorithm} & \multicolumn{2}{c|}{DDPG} & \multicolumn{2}{c|}{DDPG} & \multicolumn{2}{c}{DDPG}
     \\ \hline 
     \multicolumn{2}{l|}{ID} & Prop 4 & Prop 5 & Prop 6 & Prop 7 & Prop 8 & Prop 8
     \\ \hline 

     \multirow{2}{*}{\shortstack[c]{Network}} 
         & Activation Function
         & Tanh
         & Tanh
         & Tanh
         & Tanh
         & Tanh
         & Tanh
     \\ \cline{2-8}
         & Size
         & $2\times 20$
         & $2\times 20$ 
         & $2\times 100$ 
         & $2\times 100$ 
         & $3\times 100$ 
         & $3\times 200$ 
     \\ \hline

     
     \multirow{3}{*}{\shortstack[c]{Training \\ Time}} 
         & Reintrainer
         & $84$
         & $0$
         & $140$
         & $0$
         & $491$
         & $751$
     \\ \cline{2-8}
         & Trainify\#1
         & $304$
         & $0$
         & $\bm{25}$
         & $0$
         & $716$
         & $797$
     \\ \cline{2-8}
         & Vanilla
         & $\bm{80}$
         & $0$
         & $54$
         & $0$
         & $\bm{33}$
         & $\bm{48}$
     \\ \hline

      \multirow{3}{*}{\shortstack[c]{Timesteps}} 
         & Reintrainer
         & $\bm{3.8\times10^4}$
         & $0.0\times10^4$
         & $4.8\times10^4$
         & $0.0\times10^4$
         & $\bm{9.6\times10^3}$
         & $\bm{9.6\times10^3}$
     \\ \cline{2-8}
         & Trainify\#1
         & $7.7\times 10^4$
         & $0.0\times 10^4$
         & $\bm{1.4\times 10^4}$
         & $0.0\times 10^4$
         & $1.4\times 10^5$
         & $1.5\times 10^5$
     \\ \cline{2-8}
         & Vanilla
         & $\bm{3.8\times10^4}$
         & $0.0\times10^4$
         & $2.4\times10^4$
         & $0.0\times10^4$
         & $\bm{9.6\times10^3}$
         & $\bm{9.6\times10^3}$
     \\ \hline

      \multirow{3}{*}{\shortstack[c]{Violations}} 
         & Reintrainer
         & $256$
         & $0$
         & $128$
         & $0$
         & $\textbf{0}$
         & $\textbf{0}$
     \\ \cline{2-8}
         & Trainify\#1
         & $361$
         & $0$
         & $67$
         & $0$
         & $\textbf{0}$
         & $\textbf{0}$
     \\ \cline{2-8}
         & Vanilla
         & $\textbf{160}$
         & $0$
         & $\textbf{64}$
         & $0$
         & $\textbf{0}$
         & $\textbf{0}$
     \\ \hline


    \end{tabularx}


    \caption{Comparison of the training process of Reintrainer, Trainify and vanilla algorithms.}
    \label{tab:train_proc}
\end{table*}


